APITestGenie: Automated API Test Generation through Generative AI

Intelligent assistants powered by Large Language Models (LLMs) can generate program and test code with high accuracy, boosting developers' and testers' productivity. However, there is a lack of studies exploring LLMs for testing Web APIs, which constitute fundamental building blocks of modern software systems and pose significant test challenges. Hence, in this article, we introduce APITestGenie, an approach and tool that leverages LLMs to generate executable API test scripts from business requirements and API specifications. In experiments with 10 real-world APIs, the tool generated valid test scripts 57% of the time. With three generation attempts per task, this success rate increased to 80%. Human intervention is recommended to validate or refine generated scripts before integration into CI/CD pipelines, positioning our tool as a productivity assistant rather than a replacement for testers. Feedback from industry specialists indicated a strong interest in adopting our tool for improving the API test process.

==> Tese_Andre/abbrevs.tex <==
\chapter*{Abbreviations and Symbols}
%\addcontentsline{toc}{chapter}{Abbreviations}
\chaptermark{ABREVIATURAS E SÍMBOLOS}

\begin{flushleft}
\begin{tabular}{l p{0.8\linewidth}}
AI       & Artificial Intelligence\\
API      & Application Programming Interface\\
GPT      & Generative Pre-trained Transformers\\
HTTP     & Hypertext Transfer Protocol\\
IDE      & Integrated Development Environment\\
JSON     & JavaScript Object Notation\\
LLM      & Large Language Model\\
MVP      & Minimum Viable Product\\
NLP      & Natural Language Processing\\
OAS      & OpenAPI Specification\\
RAG      & Retrieval Augmented Generation\\
STEM     & Science, Technology, Engineering and Mathematics\\
SUT      & System Under Test\\
UI       & User Interface\\
URL      & Uniform Resource Locator\\
YAML     & Yet Another Markup Language\\

\end{tabular}
\end{flushleft}



==> Tese_Andre/abstract.tex <==
\chapter*{Abstract}
%\addcontentsline{toc}{chapter}{Abstract}

%Context

Recent advances in Large Language Models (LLMs) and generative Artificial Intelligence (AI) enabled the construction of a new generation of intelligent assistance systems that can boost the productivity of different players in the software development processes. These models have shown remarkable performance in processing natural language, which resulted in them being used for coding-related tasks, such as code generation and recommendation. Leveraging LLMs and generative AI makes it possible to use competencies in a more effective and efficient manner. Moreover, these tools make it possible to automate repetitive and time-consuming tasks.

Software testing is of the utmost importance as it fosters the quality and reliability of software products. With strict software testing procedures, companies are more secure when launching their products to the market, knowing that faulty services are unlikely to be deployed. Software testing becomes even more critical when companies develop their products' APIs. As a result of the advantages offered by API services, their adoption in modern software products has been steadily increasing. Detecting and resolving possible service bugs is essential to provide stability for the overall system.

Despite being so relevant, the creation of test cases has always been a tiresome task that demands the usage of intellectual capabilities that could be spent on developing activities. Furthermore, the growth in software products dependent on API services leads to increased time dedicated to creating tests~\cite{ref:whatIsTestAutomation}. 
Regardless of the efforts, existing techniques for automatic test generation are unable to understand the semantic information of the API due to the lack of reasoning, often falling short of achieving satisfactory relevance and completeness. 

This dissertation presents a novel approach to using generative AI to assist in the generation of relevant test case scenarios for API testing. We explore various LLMs and generative AI tools, evaluating their performance to automatically generate executable test cases that validate the application business logic. To achieve this goal, we required the definition of business requirements in natural language and contextual information specifying the services provided by an API using OpenAPI standards. This approach aligns with modern software development practices, using accessible information, and allows non-technical staff to contribute to the test generation process.
    
We developed APITestGenie, a tool validated against various API specifications and business requirement descriptions. We tested the generated outputs directly in real-world software industry scenarios, mainly provided by Critical TechWorks. Through this validation, we demonstrate the benefits of using LLMs and Generative AI to automatically generate executable API test cases. Additionally, we explore techniques and provide guidelines for using LLMs in knowledge-intensive tasks.

\chapter*{Resumo}
%\addcontentsline{toc}{chapter}{Resumo}

Avanços recentes em tecnologias como, Modelos de Linguagem de Grande Escala e Inteligência Artificial Generativa permitem a construção de uma nova geração de sistemas de assistência inteligente que podem aumentar a produtividade de diferentes intervenientes nos processos de desenvolvimento de software. Estes modelos têm demonstrado um desempenho notável no processamento de linguagem natural, resultando na sua utilização em tarefas relacionadas com geração e recomendação de código. Ao usar Modelos de Linguagem de Grande Escala e Inteligência Artificial Generativa, torna-se possível utilizar competências humanas de uma maneira mais eficaz e eficiente. Além disso, estas ferramentas permitem automatizar tarefas repetitivas e demoradas.

A testagem de software é de extrema importância, pois promove a qualidade e a fiabilidade dos produtos de software. Com procedimentos rigorosos de testagem de software, as empresas podem sentir se mais seguras ao lançar os seus produtos no mercado, sabendo que é pouco provável que serviços defeituosos sejam implementados. A testagem de software torna-se ainda mais crítica quando as empresas desenvolvem as APIs dos seus produtos. Resultado das vantagens oferecidas pelos serviços de API, a sua adoção tem vindo a aumentar nos produtos de software modernos. Detetar e resolver possíveis erros de serviço é essencial para proporcionar estabilidade a todo o sistema.

Apesar de ser tão relevante, a criação de casos de teste sempre foi uma tarefa cansativa que exige a utilização de capacidades intelectuais que poderiam ser dedicadas a atividades mais exigentes. Além disso, o crescimento dos produtos de software dependentes em serviços de API leva a um aumento do tempo dedicado à criação de testes. Independentemente dos esforços, as técnicas existentes para a geração automática de testes são incapazes de compreender a informação semântica da API e muitas vezes não conseguem alcançar uma relevância e completude satisfatórias.

Neste sentido esta dissertação apresenta uma abordagem inovadora para usar Inteligência Artificial Generativa na geração de cenários de casos de teste para a testar serviços de APIs. Exploramos vários Modelos de Linguagem de Grande Escala e ferramentas de Inteligência Artificial Generativa, avaliando o seu desempenho na geração automática de casos de teste executáveis que validam a lógica de negócios da aplicação. Para atingir esse objetivo, é necessária a definição de requisitos de negócio em linguagem natural e documentação que especifica os serviços fornecidos por uma API usando os padrões da OpenAPI. Esta abordagem está em linha com as práticas modernas de desenvolvimento de software, uma vez que utiliza informações acessíveis. Adicionalmente, permite que pessoal não técnico contribua no processo de geração de testes.

Apresentamos APITestGenie, uma ferramenta validada com várias especificações de API e descrições de requisitos de negócios. Testámos os resultados gerados diretamente em cenários reais da indústria de software, principalmente fornecidos pela Critical TechWorks. Através desta validação, procuramos demonstrar os benefícios de usar Modelos de Linguagem de Grande Escala e Inteligência Artificial Generativa para gerar automaticamente casos de teste executáveis para APIs. Além disso, exploramos técnicas e fornecemos diretrizes para a utilizar Modelos de Linguagem de Grande Escala em tarefas intensivas em conhecimento.

%Context
%Relevance
%project objectives(problem)   
%Methodology to get information
%Results 
%Conclusion



==> Tese_Andre/acknows.tex <==
\chapter*{Acknowledgements}
%\addcontentsline{toc}{chapter}{Agradecimentos}

First of all, I would like to give a special thanks to professors Bruno Lima and João Pascoal Faria for accepting the coordination of my master's thesis, as well as for their guidance in all phases of the dissertation, availability, motivation, advice, all the assessments and suggestions.

Secondly, I want to thank the opportunity to do my thesis at Critical Techworks. Thanks to the advisors Joel Martins, Ricardo Melo, Pedro Silva, and João Esteves for their follow-up and availability throughout these months. Also, thanks to the OneShop team for receiving me so well.

Lastly, I thank my colleagues Margarida Assis and Luís Viegas, who were with me on this journey and also doing their thesis.

My sincere thanks to all.

\vspace{10mm}
\flushleft{André Pereira}


==> Tese_Andre/chapter1.tex <==
\chapter{Introduction} \label{chap:intro}

The following chapter introduces the main topics explored in the context of this project. A context of the related technologies and the main points of motivation will be presented in section~\ref{sec:motivation}. Afterward, more details about the specific problem are given in section~\ref{sec:problem}, accompanied by the project's objectives in section~\ref{sec:goals}. The chapter ends with an overview of the document's structure in section~\ref{sec:structure}.

\section{Context and Motivation} \label{sec:motivation}

In recent years, the field of generative Artificial Intelligence (AI) has witnessed remarkable progress, reshaping the landscape of intelligent systems and influencing various scientific domains. Studies show that AI-powered assistants can now generate program code and test code with a high degree of accuracy based on textual prompts~\cite{ref:copilotSimpleProblems}. Very recently, organizations such as OpenAI provide out-of-the-box large language models (LLMs) like generative pre-trained transformers (GPT) pre-trained on massive amounts of data with billions of words. These tools also provide an application programming interface (API) for fine-tuning the models with task-specific training sets of much smaller size and contextual information for specialized use cases~\cite{ref:LLMfewShot}. LLM can, therefore, be used to boost the productivity of different players in the software development processes, such as developers, testers, or project managers. Through the usage of generative AI tools, it is possible to enhance productivity while optimizing the use of intellectual capabilities. 

A particular use case is software testing, a critical phase in the software development life cycle that ensures a software product's quality, reliability, and functionality. The primary goal of software testing is to identify defects or bugs in the software and ensure that it meets the specified requirements before it is released to users. Testing is an ongoing process that should begin in the early stages of development and continue throughout the software's lifecycle. Generative AI tools allow the introduction of software tests in the early stages of development or software products lacking tests, significantly increasing the system's reliability. 

The guarantees that software testing provides are of utmost importance for a product's API. Given that an API serves as a foundational component that ensures the stability of the overall system, thorough testing is exceptionally crucial. However, guaranteeing the proper functioning of API services has become substantially more challenging due to the significant surge in the number of APIs in recent years. Postman states that in 2023 it had over 121 million API collections created~\cite{ref:stateAPI2023} being that 38 million were created from 2021 to 2022~\cite{ref:stateAPI2022}. In the effort to standardize API descriptions, the OpenAPI specification has played a crucial role, a practice now widely embraced by the majority of APIs in the present day. This specification opens up an interesting way for an automated tool to interact with the system under test (SUT).

Despite all the benefits, generative AI is still little explored for test case generation in the context of more complex software systems or in the context of complex test levels, such as integration and fuzz testing. This thesis aims to not only push the boundaries of generative AI research but also address practical challenges in improving human resource efficiency and initiating the tests of software products earlier.

\section{Problem} \label{sec:problem}

Identifying and creating relevant tests for an API is a tedious and time-consuming task that consumes around 30 to 60 percent of all the product lifecycle costs~\cite{ref:testAutomation}. Additionally, this work is mostly manual as it demands careful consideration of various factors to ensure the test's effectiveness. Creating tests necessitates not only manual effort but also programming knowledge, a competency that only technical staff possess. This problem further escalates with the complexity of modern software systems. As the system grows bigger, a higher understanding is required. Current automated test generation approaches often do not meet the demands when applied to complex software systems, as they lack the depth of understanding necessary for generating meaningful test scenarios. Available solutions can generate relevant basic test types, such as unit tests focusing on code coverage. However, these types of tests have their limitations since they aim to test small components of the overall system individually.
On the other hand, integration, and system tests guarantee higher functional system integrity since they operate at a more abstract level. Nevertheless, generating these test types is more complex as they require more knowledge and a greater understanding of the system's functionalities. Despite their benefits, research falls short in addressing the automated generation of integration and fuzz tests. There is, thus, a need to break existing barriers in automated test case generation.

\section{Goals} \label{sec:goals}

The generic goal of this thesis is to explore the usage of generative AI for the automated generation of test cases.

The specific goal is to automatically generate test scripts to test the business logic of web applications through their API, simulating client applications and use cases.

For this purpose, we use as inputs:
\begin{itemize}
    \item \textbf{Business Requirements} come in the format of user stories and acceptance tests, created by nontechnical staff, describing use cases and test goals or test scenarios in natural language.
    \item \textbf{API specification}, contextual information created by technical staff documenting the API services under test specified using the OpenAPI standard.
\end{itemize}

The tool outputs are the following:
\begin{itemize}
    \item \textbf{Integration and fuzz tests} in a textual format suitable for automated execution, like an executable test script in TypeScript.
    \item \textbf{Test results}, a file containing the execution results of the generated tests.
\end{itemize}

In addition to the above, in this thesis, we expected to contribute the following:
\begin{itemize}
    \item \textbf{General-purpose LLM prompt tuned} with task-specific prompt engineering techniques.
    \item  \textbf{Knowledge-intensive LLM techniques} to adapt the solution to our task requirements.
    \item \textbf{Tool} aggregating the three outputs referred above, LLM, tests, and results to be used by non-technical staff.
    \item \textbf{Scientific paper} synthesizing relevant information collected through the thesis.
\end{itemize}

With this work, we address four research questions: 
\begin{itemize}
    \item \textbf{RQ1}: Can we effectively generate integration test cases for an API with LLM?
    \item \textbf{RQ2}: Can we effectively generate fuzz test cases for an API with LLM?
    \item \textbf{RQ3}: How can prompt-tuned models compare to achieved baseline results?
    \item \textbf{RQ4}: Can the industry use the proposed solution to improve resource efficiency?
\end{itemize}

This thesis relies on an academia-industry collaboration involving FEUP and Critical TechWorks. Critical Techworks~\cite{ref:CTW} is a software house at the forefront of automotive innovation, collaborating with the BMW Group to transform the future of motion. This collaboration allows us to validate the solution with real-world use case scenarios provided by Critical TechWorks.

\section{Document Structure} \label{sec:structure}

In addition to this introduction, this document is divided into four chapters. Chapter~\ref{chap:back&sa} reviews the state-of-the-art key research areas related to the thesis: generative AI, API, and automated testing. 
Chapter~\ref{chap:solut} explains the APITestGenie architecture designed to solve the highlighted problems, emphasizing the technologies used, data processing, and prompt engineering techniques, and showcasing an initial prototype.
Chapter~\ref{chap:results} details the validation process, covering the setup, results collection, key conclusions, and limitations encountered.
Lastly, Chapter~\ref{chap:concl} presents some related work, accompanied by a final discussion on the expectations for the project.

==> Tese_Andre/chapter2.tex <==
\chapter{Background and State of The Art} \label{chap:back&sa}

This chapter provides an overview of the existing literature and practices about topics used throughout the project. First, section~\ref{sec:LLM} explains the concept of generative AI and LLM, how LLM works, and how these models are used. The key benefits, challenges, and a list of the most relevant LLM tools are also presented with their value proposition. Section~\ref {sec:API} explains what a Web API is, followed by an introduction to existing specification standards and trending ways to test them, exploring the topic of test automation.
%Lastly, in section~\ref{sec:discussion}, a summary highlighting emerging topics is provided.

\section{Generative AI and Large Language Models} \label{sec:LLM}

As some sources state, programmers and non-programmers have long dreamed of being able to provide a computer with natural-language instructions and have the machine handle it. The potential benefits in productivity and creativity resulting from this are noteworthy~\cite{ref:generativeAIvsLLM}. This was made possible by Generative AI and LLM. In this section, we describe what each of the terms means. Of the two, Generative AI is broader, whereas LLM is more specific.

% Description of Generative AI
\subsection{What is Generative AI?}

Generative AI is a more general term that refers to artificial intelligence models that have the capability to generate content. The content can vary between text, code, images, video, music, and more~\cite{ref:whatIsLLM}. %~\hyperfootnote{https://www.elastic.co/what-is/large-language-models}{foot:whatIsLLM}. 
%Examples of generative AI include Midjourney, DALL-E, and ChatGPT
Any machine learning model capable of dynamically creating output after training can be called Generative AI.
The ability to generate complex forms of output is what distinguishes generative AI from other more straightforward types of machine learning that make predictions based on new data entries~\cite{ref:generativeAIvsLLM}.%~\hyperfootnote{https://quiq.com/blog/generative-ai-vs-large-language-models/}{foot:generativeAIvsLLM}

%Generative AI for coding
%\subsubsection{Generative AI for coding}
 
In the context of this project, the most relevant type of Generative AI is code generation. 
Code-generation tools are usually trained on massive amounts of data, after which they can take simple prompts and produce code. It is possible to ask to write a function that converts between several different coordinate systems, create a web app, or translate from Python to Javascript.
As things stand now, the code often needs to be completed in small ways. For example, it might produce a function that takes an argument as input that is never used or lacks a return function. 
However, some software developers are using this model to automate substantial portions of their work, to understand new codebases with which they're unfamiliar, or to write comments and unit tests~\cite{ref:generativeAIvsLLM}.%~\footref{foot:generativeAIvsLLM}

%What is LLM
\subsection{What is a LLM?}

LLMs are a particular type of generative AI trained on text that is capable of producing textual content. This implies that all LLMs are generative AI models.

A LLM is a deep learning algorithm that can perform various natural language processing tasks. The main component of an LLM is its transformer model, which is trained using massive data sets. This enables LLM to recognize, translate, predict, or generate text, code, and other content. LLMs are commonly compared to neural networks~\cite{ref:whatIsLLM}, computing systems inspired by the human brain. These neural networks work using a network of layered nodes like neurons. The most critical capability of LLM is its capacity to teach human languages to AI applications~\cite{ref:whatIsLLM}.%~\footref{foot:whatIsLLM}
In the context of this thesis, LLMs are used to perform various tasks, such as understanding structures and writing software code.

The transformer model, previously introduced, consists of an encoder and a decoder. Both components are responsible for processing the data by tokenizing it and simultaneously conducting mathematical equations to discover relationships between tokens~\cite{ref:whatIsLLM}. %~\footref{foot:whatIsLLM}.
A token is a sequence of characters in a particular document grouped as a meaningful semantic unit for processing. The goal of tokenization is to effectively attain rare words in a model's vocabulary while maintaining a limited number of tokens per sequence in the interest of computational complexity~\cite{ref:challengesLLM}. %All this processing is why AI applications can detect patterns a human would see if given the same query.

%Tokenization is the process of breaking a sequence of words or characters into smaller units called tokens so they can be fed into the model. One common tokenization approach is subword tokenization, where we split words into smaller units called subwords or WordPieces~\cite{ref:challengesLLM}.

In addition to the transformer model, LLMs are composed of multiple neural network components. See figure~\ref{fig:LLMStructure}. The most relevant ones are:
\begin{itemize}
    \item The input and output embedding component create embeddings from the received tokens. Embeddings are a way to represent a word in a numeric vector. Words with similar meanings have very close vectorial representations. This part of the LLM captures the semantic and syntactic meaning of the text so that the model can understand the context~\cite{ref:whatIsLLM}.%~\footref{foot:whatIsLLM}.
    \item The feed-forward component comprises multiple fully connected layers that transform the input embeddings, allowing the model to figure out more complex patterns. These layers enable the model to gather higher-level abstractions that allow the LLM to understand the user's intent with the text input~\cite{ref:howLLMWork}.%~\hyperfootnote{https://blog.gopenai.com/how-transformers-and-large-language-models-llms-work-3f20bb41c1ff}{foot:howLLMWork}.
    \item The positional encoding component interprets and remembers a sequence of tokens in the input text. This allows the LLM to capture the relationship between tokens in a sentence~\cite{ref:whatIsLLM}.%~\footref{foot:whatIsLLM}.
    \item The attention mechanisms enable the LLM to focus on single parts of the input text that are relevant to the task at hand. It also creates a context-aware representation of each token, getting both its meaning and its relationship to other words in the input. This component allows the generation of the most accurate outputs~\cite{ref:howLLMWork}.%~\footref{foot:howLLMWork}.
\end{itemize}

\begin{figure}[h]
    \includegraphics[width=0.80\textwidth]{figures/LLMStructure.pdf}
    \caption[Structure of Large Language Models]{Structure of Large Language Models~\cite{ref:howLLMWork}.%~\footref{foot:howLLMWork}
    }
    \label{fig:LLMStructure} 
\end{figure}

%LLM can be distinguished into three main kinds:
%\begin{itemize}
 %   \item Generic or raw language models predict the next word based on the language in the training data. These language models perform information retrieval tasks.
  %  \item Instruction-tuned language models are trained to predict responses to the instructions given in the input. This allows them to perform sentiment analysis or to generate text or code.
   % \item Dialog-tuned language models are trained to have a dialog by predicting the subsequent response. Think of chatbots or conversational AI.
%\end{itemize}\cite{ref:whatIsLLM}

% How LLM work 
%\subsubsection{LLM training}

In addition to the complex internal components that an LLM processes, it also needs to be trained to receive a text input and generate an output prediction. This training can be done in three different ways:

%But before a large language model can receive text input and generate an output prediction, it requires training to fulfill general functions and finetuning, enabling it to perform specific tasks.
\begin{enumerate}
    \item Pretraining: In this phase, LLMs are trained using large textual data sets from websites like Wikipedia\hyperfootnote{https://en.wikipedia.org/wiki/Main_Page}{foot:wikipedia}, GitHub\hyperfootnote{https://github.com/}{foot:github}, or others. These data sets consist of trillions of words, and their quality affects the language model's performance. At this stage, the LLM engages in unsupervised learning, meaning it processes the data sets fed to it without specific instructions. During this process, the LLM's algorithm learns how words relate and their meaning in different contexts. %For example, it would learn to understand whether "right" means "correct" or the opposite of "left."
    \item Finetuning: The LLM is trained on smaller, more task-specific data sets. In this phase, the internal representation of the words is adjusted to the specific task, thus optimizing the model performance for the task at hand. In the case of automated test generation, a model could be fine-tuned with a set of high-quality tests. A key challenge of finetuning chatbots is creating a broad training dataset of high-quality conversations. To address this problem, it is possible to use existing LLMs to generate high-quality synthetic conversation datasets based on a small number of expert-written examples~\cite{ref:challengesLLM}.
    % Finetuning all LLMs requires the same amount of memory as pretraining, rendering it infeasible for many practitioners. \cite{ref:challengesLLM}
    \item Prompt-tuning: This is similar to finetuning, where the model is trained to perform a specific task. However, this training is done by either few-shot prompting or zero-shot prompting~\cite{ref:whatIsLLM}. A prompt is a text input given to an LLM. Few-shot prompting teaches the model to predict outputs through the use of examples. This is done by associating a given prompt with its expected output. Alternatively, zero-shot prompting formulates the prompt without examples attempting to take advantage of the LLM reasoning patterns.%~\footref{foot:whatIsLLM}.
\end{enumerate}


%Promptuning ------Few-shot prompting------
%Customer review: This plant is so beautiful!
%Customer sentiment: positive

%Customer review: This plant is so hideous!
%Customer sentiment: negative

%----Zero-shot prompting------
%The sentiment in 'This plant is so hideous' is…


% How are they being used
\subsection{Use cases}

Even though many impactful LLMs have just completed their first year of deployment, they are already used in numerous business applications. This exhibits the relevance that such models have. Of these applications, the most relevant use cases in the context of this project are~\cite{ref:whatIsLLM}.%~\footref{foot:whatIsLLM}:
\begin{itemize}
    \item Information retrieval: This refers to using LLM to retrieve, summarize, and communicate information. Due to the vast knowledge base that an LLM possesses, it can respond to a query with both recurrent and unique scenarios.
    %Whenever you use their search feature, you rely on a large language model to produce information in response to a query. It can retrieve information then summarize and communicate the answer in a conversational style.
    \item Code generation: Code generation refers to using an LLM to output new code for a given specification or problem provided as a prompt. Several computer programming-specific LLMs and approaches have been proposed~\cite{ref:challengesLLM}. A code generation solution based on a query text and an API specification is presented in Figure~\ref{fig:apiUseCase}. In this solution the author first inputs the LLM with the API specification describing the available functions. Then it sends a prompt requesting to generate a program for a given problem based on the API specification. The LLM then generates a program that can be validated with the API specification.

\begin{figure}[h!]
    \includegraphics[width=0.60\textwidth]{figures/apiUseCase.pdf}
    \caption[LLM prompting with API specification.]{LLM prompting with API specification.~\cite{ref:challengesLLM}}
    \label{fig:apiUseCase} 
\end{figure}
    
    \item Conversational AI: LLMs can maintain a conversational engagement with the person making the prompts. This is done by keeping a context of the current chat and interpreting the meaning of the consecutive queries. After multiple interactions, a response with more complete and improved information is answered. 
    %\item Text generation: Large language models behind generative AI, like ChatGPT, can generate text based on inputs. They can produce an example of text when prompted. For example: "Write me a poem about palm trees in the style of Emily Dickinson."
    %\item Sentiment analysis: As applications of natural language processing, large language models enable companies to analyze the sentiment of textual data.
    \item Creative work: LLMs can generate stories and scripts. When used in long-form generations, their inability to keep the entire generated work within context creates the need to provide modular prompts, see Figure~\ref{fig:modularPrompt}. In the provided example in module 1 the user first starts by making a broader request, for example a paragraph outline for a novel. Then in module 2 the user request iteratively a more specific task, taking in consideration the output of the general one, for example, the user requests to create a text draft for each of the paragraph. This process can continue as needed or can be finalized. In the example, module 3 is finalized with a request to validate the generated output. 
    For smaller and more general creative tasks, LLMs have a good capacity for generating ideas.

\begin{figure}[h]
    \includegraphics[width=0.45\textwidth]{figures/modularPrompt.pdf}
    \caption[Modular Prompting]{Modular Prompting~\cite{ref:challengesLLM}}
    \label{fig:modularPrompt} 
\end{figure}

\end{itemize}

With such a variety of use cases, LLM can be found in fields such as Technology and Management, as seen in~\cite{ref:challengesLLM}. Both are highly relevant to the problem of software testing at hand.

% benefits
\subsection{Benefits}

LLM provides increasing benefits of adoption due to its capacity for problem-solving. It provides information in comprehensive and diversified ways that are easy for users to understand. Some other advantages of using LLM are:
\begin{itemize}
    %\item Large set of applications: They can be used for language translation, sentence completion, sentiment analysis, question answering, mathematical equations, and more.
    \item Always improving: LLM performance continually improves as more data and parameters are added to its training. In other words, the more it learns, the better it gets. What's more, LLMs are capable of in-context learning. Once an LLM has been pre-trained, prompt-tuning enables the model to learn from the prompt without additional parameters. In this way, the model is continually learning~\cite{ref:whatIsLLM}.%~\footref{foot:whatIsLLM}.
    %\item Learn fast: When demonstrating in-context learning, LLMs learn quickly because they do not require additional weight, resources, and parameters for training. It is fast in the sense that it does not need too many examples.
    \item Scale: The scale of the LLMs provides a high degree of stability and predictability. This trend is expected to develop even further for larger models, making them more robust and capable of learning from a few training examples~\cite{ref:understandLLM}.
    \item Provide skills: LLM enables people to rapidly obtain a broad set of skills they do not have. This can be, for instance, some non-programmers asking a LLM to generate code for a given situation. Furthermore, some jobs can be automated using LLM~\cite{ref:understandLLM}. 
    
\end{itemize}

% Challenges 
\subsection{Challenges}

LLMs might give us the impression that they understand the meaning and can respond accurately. However, they remain a technological tool and, as such, lack intrinsic human characteristics, criticism, and causality. 
The output of a LLM is only based on probabilities, thus facing various challenges. Some of them are explored below:

\begin{itemize}
    \item Hallucinations: When an LLM produces a false output or does not match the user's intent. Since LLMs predict the next syntactically correct word or phrase, they can't fully interpret human meaning~\cite{ref:whatIsLLM}. %~\footref{foot:whatIsLLM}. 
    This also relates to the fact that LLMs do not understand what is being asked of them. This lack of understanding causes them to perform well in most cases while performing poorly on important inputs~\cite{ref:understandLLM}. Hallucinations can either be intrinsic or extrinsic. When intrinsic, the generated text logically contradicts the source content. If extrinsic, we cannot verify the output correctness from the provided source~\cite{ref:challengesLLM}. Users who lack knowledge of the task subject can be highly influenced by model hallucinations, as they would not be able to verify the accuracy of the responses.
    \item Prompt Brittleness: The prompt syntax and semantics can significantly impact the model output. Consequently, slight variations to the input query may result in dramatic output changes~\cite{ref:challengesLLM}. This is highly related to prompt engineering explored in section~\ref{sec:promptEng}.
    \item Security: LLMs present substantial security risks when not managed or surveilled properly. They can leak people's private information, participate in phishing scams, and produce spam. Users with malicious intent can reprogram them to their ideologies or biases and contribute to the spread of misinformation~\cite{ref:whatIsLLM}. %~\footref{foot:whatIsLLM}. 
    Due to their extensive capabilities, it is challenging to ensure the safety of the people and society~\cite{ref:understandLLM}. Companies also face challenges when using these tools to maintain data privacy since LLMs use all the data they can access. Therefore, performing tasks that require sensitive information that must not be publicly available becomes impossible. 
    \item Bias: The data used to train the LLM will affect the model's outputs. As such, if the data lacks diversity, the results produced by the LLM will only consider the particular information~\cite{ref:whatIsLLM}. %~\footref{foot:whatIsLLM}. 
    This may lead to generating outputs not well-aligned with human values or intentions, which can have unintended or negative consequences~\cite{ref:challengesLLM}. Some studies suggest that a human should always be integrated into the loop of text generation~\cite{ref:understandLLM}. However, due to the size of the datasets, it is impractical for any individual to read or conduct quality assessments on all documents\cite{ref:challengesLLM}. % Miss-alignments of the model objectives with human values \cite{ref:understandLLM}
    \item Consent: LLMs are trained on trillions of data sets, some of which might not have been obtained consensually. When scraping data from the internet, LLMs have been known to ignore copyright licenses, plagiarize written content, and use proprietary content without getting permission from the original owners or artists. When it produces results, there is no way to track the origin of the data, and often, no credit is given to the creators, resulting in copyright infringements~\cite{ref:whatIsLLM}. %~\footref{foot:whatIsLLM}.
    \item Deployment: LLMs work with enormous quantities of data, and as such, it can be difficult, time-demanding, and resource-consuming to deploy and maintain LLMs~\cite{ref:understandLLM}. Training a single LLM can require hundreds of thousands of compute hours, costing millions of dollars in computing power and energy~\cite{ref:challengesLLM}.
    \item Outdated knowledge: Factual information learned during pretraining can become inaccurate or outdated as time passes. Updating isolated model behavior or factual knowledge can be expensive and untargeted, which might cause unintended side-effects~\cite{ref:challengesLLM}.
    \item Tasks not solvable by scale: Refers to the model's inability to improve in some specific tasks. For instance, in inverse scaling tasks, the performance worsens as the model scales. Compositional tasks are also related to the problem as they are composed of multiple sub-problems and require the models to go beyond rote memorization of observed facts to deduce novel knowledge~\cite{ref:challengesLLM}.
\end{itemize}

% Improvement methods 
\subsection{Improvement techniques} \label{sec:improvement}
Some literature suggests some techniques that may be used to improve the LLM output. This may lead the model to reach state-of-the-art downstream performances~\cite{ref:challengesLLM}. Some of these techniques are: 
\begin{itemize}
    \item Instruction Finetuning: Finetune pre-trained LLM on instructional data. The provided data should contain natural language instructions and the desired responses according to human judgment.
    \item Reinforcement Learning From Human Feedback: Works by using a pre-trained LLM to generate text, which is then evaluated by humans, for example, ranking two model generations for the same prompt. This data is then collected to learn a reward model that predicts a scalar reward given any generated text. The reward captures human preferences when judging model output. Finally, it is possible to optimize the LLM against such a reward model using reinforcement learning algorithms.
    \item Self-improvement: Improve the LLM with self-generated data. Iteratively prompt the model to generate rationales and then finetune them on those leading to correct answers.
\end{itemize}

Evol-Instruct prompts for code is a concrete use case of a self-improvement technique that has proven its effectiveness~\cite{ref:wizardcoder}. It uses an evolutionary approach to attempt to make code instructions more complex to enhance the finetuning effectiveness of LLMs pre-trained on code. Figure~\ref{fig:promptTemplate} displays the suggested code evolutionary prompt template.

\begin{figure}[h]
    \begin{lstlisting}[style=txt]
Please increase the difficulty of the given programming test question a bit.

You can increase the difficulty using, but not limited to, the following methods:
{method}

{question}
    \end{lstlisting}
    \caption[Code evolutionary prompt template]{Code evolutionary prompt template~\cite{ref:wizardcoder}}
    \label{fig:promptTemplate}
\end{figure}

In Figure~\ref{fig:promptTemplate} \textit{{question}} represents the current code instruction awaiting evolution, and \textit{{method}} is the type of evolution. The five types are the following, see Figure~\ref{fig:evolutionTypes}.

\begin{figure}[h]
    \begin{lstlisting}[style=txt]
Add new constraints and requirements to the original problem, adding approximately 10 additional words.

Replace a commonly used requirement in the programming task with a less common and more specific one.

If the original problem can be solved with only a few logical steps, please add more reasoning steps.

Provide a piece of erroneous code as a reference to increase misdirection.

Propose higher time or space complexity requirements, but please refrain from doing so frequently.
    \end{lstlisting}
    \caption[Evolution Types]{Evolution Types~\cite{ref:wizardcoder}}
    \label{fig:evolutionTypes}
\end{figure}

The Evol-Instruct technique is intended to be iteratively employed on a dataset to produce evolved data. After each round of data evolution, the evolved data is then merged with all previous rounds into the original dataset to finetune the model.

TELeR taxonomy~\cite{ref:teler} presents prompt design properties that increase the performance of LLMs in a wide range of complex tasks. Figure~\ref{fig:teler} summarizes the properties presented in the TELeR taxonomy.
\begin{figure}[h!]
    \centering
    \includegraphics[width=.9\linewidth]{figures/teler.pdf}
    \caption[TELeR Prompt Taxonomy]{TELeR Prompt Taxonomy~\cite{ref:teler}.}
    \label{fig:teler}
\end{figure}
They categorize LLM prompts along four different dimensions:
\begin{itemize}
    \item \textbf{Turn}: Number of turns used while prompting LLM, singe, or multi-turn. Explore in more detail in Section~\ref{sec:promptEng}.
    \item \textbf{Expression}: Style of the overall directive and the associated sub-tasks, either question-style or instruction-style.
    \item \textbf{Role}: System role is defined in the LLM and can be categorized as either system-role defined or undefined.
    \item \textbf{Level of Details}: Degree of detail provided in the prompt, divided into seven distinct levels. Figure~\ref{fig:teler} clearly identifies the contents of each prompt level.
\end{itemize}

\subsection{Prompt Engineering}\label{sec:promptEng}

Designing natural language queries that steer the model's outputs toward desired outcomes is often called prompt engineering. There are lots of equally plausible prompting techniques, and the current state of prompt engineering still requires lots of experimentation. There is little theoretical understanding of why a particular way to phrase a task achieves better empirical results. Developing LLMs that are robust to prompt styles and formats remains unsolved, leaving practitioners to design prompts ad-hoc rather than systematically~\cite{ref:challengesLLM}. Existing prompt engineering methods can be distributed in two main classes, single-turn and multi-turn prompting, using single-shot and multi-shot techniques, respectively. Single-shot techniques are based on a single prompt input, while multi-shot techniques require multiple prompt inputs.

% Mode details in Page 18-20 figure 6
Example of single-turn prompting techniques~\cite{ref:challengesLLM} are:
\begin{itemize}
    \item In-Context Learning: Ability to learn a new task only via inference.
    \item Instruction-Following: Append task-describing instructions at the beginning of the input prompts.
    \item Chain-of-Thought: Construct a series of intermediate reasoning steps that lead to the final output.
    \item Impersonation: Ask the model to pretend to be a domain expert when answering a domain-specific question.
\end{itemize}

Example of Multi-turn prompting techniques~\cite{ref:challengesLLM} are:
\begin{itemize}
    \item Ask-Me-Anything: Uses multiple prompt templates, which are used to reformat few-shot example inputs into an open-ended question-answering format. The final output is obtained by aggregating the LLM predictions for each reformatted input via a majority vote.
    \item Self-Consistency: Extends chain-of-thought prompting by sampling multiple reasoning paths and selecting the most consistent answer via a majority vote.
    \item Least-To-Most: Uses a set of constant prompts to use the LLM to decompose a given complex problem into a series of subproblems. The LLM sequentially solves the subproblems with prompts for later-stage subproblems containing previously produced solutions, iteratively building the final output.
    \item Automatic Reasoning and Tool-Use: Method to automatically generate multi-step reasoning prompts, including symbolic calls to external tools such as search and code generation or execution. This allows the retrieval of demonstrations of related tasks from a library of tasks accompanied by their reasoning steps. It also uses a frozen language model to generate intermediate reasoning steps.
    \item Self-Refine: Based on the notion of iterative refinement, the LLM generates an initial output and then iteratively provides feedback on the previous output, followed by a refinement step in which the feedback is incorporated into a revised output.
    \item Tree of Thoughts: Generalizes chain of thought to maintain a tree of thoughts, where each thought is a language sequence that serves as an intermediate step. Doing so enables the LLM to self-evaluate intermediate thoughts' progress toward solving the problem. It is then possible to incorporate search algorithms, such as breadth-first or depth-first search, allowing systematic exploration of the tree with lookahead and backtracking.
\end{itemize}

It is possible to build a system that accesses external knowledge sources for more complex and knowledge-intensive tasks. This enables factual consistency, improves reliability and transparency of the generated responses, and helps to keep the data up to date~\cite{ref:RAG}. Meta AI researchers introduced Retrieval Augmented Generation (RAG)~\cite{ref:RAGKnowldegeIntensive}, a method for knowledge-intensive tasks. RAG takes an input and retrieves a set of relevant or supporting documents from a source. The documents are concatenated in context with the original input prompt and fed to the text generator, which produces the final output. This makes RAG adaptive for situations where facts could evolve over time. This is very useful as LLM parametric knowledge is static. RAG allows language models to bypass retraining, enabling access to the latest information for generating reliable outputs via retrieval-based generation. RAG internal knowledge can be modified efficiently and without retraining the entire model. 

% Evaluation 
\subsection{Evaluation Metrics}

The number of LLMs available to use has been increasing throughout the previous years. This motivated the research community to create multiple text-based benchmarks covering reasoning, reading comprehension, science, technology, engineering and mathematics (STEM), and coding~\cite{ref:gemini}. By measuring these benchmarks, it is possible to compare distinct LLMs effectively. However, due to the novelty of the subject and the lack of standardization, some models have not been tested against some of the benchmarks. Benchmarks that are widely used and related to code and reasoning tasks are considered in the context of this project. The following list aims to present and explain the benchmarks used in this thesis: 

\begin{itemize}
    \item MMLU: Measures a text model's multitask accuracy. The test covers 57 tasks, including elementary mathematics, US history, computer science, law, and more. To attain high accuracy on this test, models must possess extensive world knowledge and problem-solving ability~\cite{ref:mmlu}.
    \item HumanEval: Assess language comprehension, reasoning, algorithms, and simple mathematics on a set of 164 handwritten programming problems. The dataset aims to evaluate the model's functional correctness and measure the problem-solving capabilities of their models~\cite{ref:humanEval}.
    \item Natural2Code: Python code generation tasks without web leakage~\cite{ref:gemini}. 
    \item DROP: Discrete Reasoning Over Paragraphs is a crowdsourced, adversarially-created, 96k-question benchmark in which a system must resolve references in a question regarding multiple input positions and perform discrete operations over them such as addition, counting, or sorting~\cite{ref:drop}.
    \item pass@k: Gives the probability that at least one correct sample is generated in the first k attempts for solving a coding task. The unbiased estimator, see Equation~\ref{eq:pass@k}, can be used to minimize the variance inherent to the LLMs~\cite{ref:humanEval}.
    \begin{equation}
        pass@k = 
        \begin{cases}
        1 - \frac{\binom{n-c}{k}}{\binom{n}{k}} & \text{if } n - c \ge k \\
        1 & \text{if } n - c < k \\
        \end{cases}
        \label{eq:pass@k}
    \end{equation}
\end{itemize}

%Popular LLMs
\subsection{Popular Tools}

LLMs have attracted many people's attention, resulting in high adoption across several industries. However, due to their billions of parameters and model size, LLMs have a large memory footprint, making them unfit for single-device memory. They also required scaling across GPUs and compute nodes, which indulges in communication and synchronization costs~\cite{ref:challengesLLM}. Due to these constraints, readily available LLM tools can be handy. Table~\ref{tab:LLMTools} lists most popular state-of-the-art LLM tools with their related benchmarks.

\begin{table}[h]
\scalebox{0.95}{
  \begin{tabular}{c|c|c|c|c|c|c|c}
    \textbf{} & \textbf{GPT-4} & \textbf{GPT-3.5} & \textbf{Gemini
Pro} & \textbf{PaLM 2-L} & \textbf{Grok} & \textbf{LLAMA-2} & \textbf{Claude 2} \\\hline
    Company & OpenAI & OpenAI & Google & Google & xAI & Meta & Anthropic \\
    MMLU & 87\% & 70\% & 79\% & 78\% & 73\% & 68\% & 79\%  \\
    HumanEval & 67\% & 48\% & 68\% & - & 63\% & 30\% & 70\%  \\
    Natural2Code & 74\% & 62\% & 70\% & - & - & - & -  \\
    DROP & 81\% & 64\% & 74\% & 82\% & - & - & - \\
  \end{tabular}
}
\caption[Large language model tools]{Large language model tools. Metric values extracted from~\cite{ref:gemini}.}
\label{tab:LLMTools}
\end{table}

OpenAI's text generation models, GPT-4 and GPT-3.5, have been trained to understand natural and formal language. They can both be used in a wide variety of tasks, including content or code generation, summarization, conversation, creative writing, and more~\cite{ref:openAI}. %~\hyperfootnote{https://platform.openai.com/docs/overview}{foot:openAI}. 
GPT-4 distinguishes itself from GPT-3.5 as it is a multimodal model with better performance and can accept image inputs~\cite{ref:gpt4Report}. Currently, these models can be used through OpenAI API, which allows direct calls to the model. The ChatGPT chatbot is also available, where it is possible to send text requests. Or through assistants, entities embedded within a context window capable of performing tasks for users. Additionally, with the premium subscription, it is possible to create GPTs, a custom ChatGPT version that combines instructions, extra knowledge, and skills to address a specific purpose.

Gemini is a newly introduced multimodal LLM developed by Google, which means that it can operate across and combine different types of information, including text, code, audio, image, and video. Gemini comes in three different sizes, nano, pro, and ultra, allowing it to run efficiently on everything from mobile devices to data centers. Currently, the only way to use Gemini Pro is through Google chatbot Bard~\cite{ref:geminiIntroduction}. %~\hyperfootnote{https://blog.google/technology/ai/google-gemini-ai/}{foot:geminiIntroduction}.
Gemini Ultra is also a model worth mentioning, as it outperforms all the other LLMs in most of the benchmarks~\cite{ref:gemini}. However, it is not expected to be available for public use during the length of this project.

Palm2 is a model capable of advanced reasoning tasks, including code and math, classification and question answering, translation and multilingual proficiency, and natural language generation. It is an improved version of Palm that brings together compute-optimal scaling, an improved dataset mixture, and model architecture improvements~\cite{ref:palm2}. %~\hyperfootnote{https://ai.google/discover/palm2/}{foot:palm2}. 
Palm2 is not readily available to use as it was the predecessor of Gemini in the Bard chatbot.

Grok's primary goal is to engage with the users in a conversational manner. A unique advantage of Grok is that it is fed on real-time data of the world via the X platform~\hyperfootnote{https://twitter.com/}{foot:x}. It is expected to answer distinct questions rejected by other models. As the developers state, Grok is also designed to have a bit of wit and a rebellious streak. Currently, Grok is only available to a limited number of users in the United States~\cite{ref:grok}.%~\hyperfootnote{https://x.ai/}{foot:grok}.

Llama2 created by Meta comprises two distinct models, Llama Chat, a chatbot, and the Code Llama trained for code generation. It is available in sizes ranging from 7 billion to 70 billion parameters. Currently, Llama2 is available for free usage for research and commercial purposes~\cite{ref:llama2}. %~\hyperfootnote{https://ai.meta.com/llama/}{foot:llama2}. 
Shortly after Llama2 open release, the open-source community tried to finetune it and immediately achieved a new top score. At first, the community created the Phind 34B Python model with a HumanEval score of 70\%, which was finetuned on a custom dataset of about 80,000 high-quality programming tasks and solutions. More recently, WizardCoder-34B~WizardCoder~\hyperfootnote{https://github.com/nlpxucan/WizardLM/tree/main/WizardCoder}{foot:wizard} presented a score of 73\% in the first pass of HumanEval, making it one of the most capable open-source LLM available~\cite{ref:wizardcoder}. Most of the open source models can be found in Hugging Face~\hyperfootnote{https://huggingface.co/}{foot:huggingFace}, a platform where the machine learning collaborates on models, datasets, and applications.

Claude 2 is an easy to converse model that clearly explains its thinking, is unlikely to produce harmful outputs, and has a large memory. This model, introduced in July 2023, is an upgraded version of Claude with improved performance and more extended responses. It can be accessed via API and a chatBot~\footnote{\url{https://claude.ai/}}. A key feature of Claude 2 is its capacity to receive up to 100k tokens in each prompt, making it the model with the larger context size. The closest is GPT-4 with 32k tokens of context size. This allows Claude 2 to work over hundreds of pages of technical documentation. Claude also has good coding skills, as seen through the scores acquired in the HumanEval metric, see Table~\ref{tab:LLMTools}, outperforming all the other LLMs. Claude 2 has proven capable of going head-to-head with other state-of-the-art models in various use cases, making it gain multiple business clients. A big problem with Clause 2 is that it is not yet available in all regions. This includes Portugal, the country where the majority of the work for this project will be done. Therefore, accessing Claude 2 would pose challenges not intended in the project's scope. Nevertheless, Claude 2 is a model worth looking for~\cite{ref:claude2}.%~\hyperfootnote{https://www.anthropic.com/news/claude-2}{foot:claude2}.

Considering the benchmarks in Table~\ref{tab:LLMTools} and the capabilities of each model, it is possible to conclude that some of the models are best suited to solve the problem at hand. These are GPT-4, GPT-3.5, Gemini Pro, Claude2 and WizardCoder. We will focus the research on openAI models, GPT-4 and GPT-3.5, since their capabilities align better with the ones that we expect from a model to be used in a business context while also having an excellent performance in state-of-the-art metrics. They are also readily available from the same interface and provide many customization options. 

More specific tools related to code generation and suggestions in real-time are also available. These tools use LLMs, like the one listed in Table~\ref{tab:LLMTools}, to generate their code suggestions. Table~\ref{tab:CodeTools} lists the most relevant tools, comparing them using the HumanEval dataset. The code quality metrics considered are validity, correctness, reliability, and maintainability. Validity verifies if any errors were raised during the execution of the code. Correctness is calculated using the number of passed tests divided by all tests. This allows us to calculate the success percentage of the code for each problem. Reliability considers the total number of bugs found in the code. Maintainability analyses the existing code smells in the code and estimates the time to fix them~\cite{ref:codeToolsBenchmarks}.

\begin{table}[h]
  \begin{tabular}{c|c|c}
    \textbf{} & \textbf{Github Copilot} & \textbf{CodeWhisperer} \\ \hline
    Company & GitHub & Amazon \\
    Validity & 91.5\% & 90.2\% \\
    Correctness & 59.9\% & 52.0\% \\
    Reliability & 3 & 1 \\
    Maintainability & 172m & 117m \\ 
  \end{tabular}
  \caption[Evaluation of code generation tools.]{Evaluation of code generation tools. Based on humanEval~\cite{ref:codeToolsBenchmarks}.}
  \label{tab:CodeTools}
\end{table}

GitHub Copilot is an AI pair programmer that offers autocomplete-style suggestions while coding. It can interpret initial and incomplete code snippets or natural language comments describing the purpose of the code. GitHub Copilot analyzes the context of the file and related files to offer suggestions in the text editor. It is powered by a generative AI model developed by GitHub, OpenAI, and Microsoft, trained on all languages available in public repositories. Its performance varies depending on the volume and diversity of training data available for the specific language. Currently, GitHub Copilot is available as an extension for multiple widely used integrated development environments (IDEs)~\cite{ref:copilot}.%~\hyperfootnote{https://docs.github.com/en/copilot/overview-of-github-copilot/about-github-copilot-individual}{foot:copilot}.

Amazon CodeWhisperer is a general-purpose, machine learning-powered code generator that provides code recommendations in real time. As the user writes code, CodeWhisperer automatically generates suggestions based on existing code and comments. The model can give multiple recommendations that the user can cycle through. These recommendations can vary in size and scope, ranging from single-line comments to fully formed functions. CodeWhisperer can also scan the code to highlight and define security issues. Currently, it is available to use as an extension in multiple IDEs.
~\cite{ref:whisperer}.%~\hyperfootnote{https://docs.aws.amazon.com/codewhisperer/latest/userguide/what-is-cwspr.html}{foot:whisperer}

%- TODO CodeGen https://github.com/salesforce/CodeGen?tab=readme-ov-file

These code-generating tools are very useful in enhancing a developer's productivity. They can generate useful suggestions by interpreting the context window where the development is being made. However, to make use of these tools, the users need to have some prior knowledge related to software and code development since it is necessary for them to know how to use an IDE, the only place where these tools are available. Therefore, nontechnical staff would require some training to use these tools.

\subsection{OpenAI API}

The OpenAI API provides a simple interface composed of multiple endpoints allowing developers to create an intelligence layer in their applications powered by OpenAI's state of the art models like GPT-4 or GPT-3.5. To start making requests, the developer first needs to create an OpenAI account and a secret key that must be sent with every request. This key, on top of serving as a security mechanism, allows the OpenAI system to link the requests to the respective account. Currently, there are three languages that can be used to perform requests curl, python, and node.js. For the last two, a custom library is available, which makes working with Python and node.js simple and efficient~\cite{ref:openAI}. 

One of the available endpoints is the chat completions API~\hyperfootnote{https://platform.openai.com/docs/guides/text-generation/chat-completions-api}{foot:chatCompletion}. Chat models take a list of messages as input and return a model-generated message as output. An example of a chat completion API call in Python looks like the following, see Figure~\ref{fig:chatCompletion}.

\begin{figure}[h]
    \lstinputlisting[style=python]{./code/chatCompletionCall.py}
    \caption[Chat completion Python request]{Chat completion python request~\cite{ref:openAI}}
    \label{fig:chatCompletion}
\end{figure}

There are two important inputs in the example of Figure~\ref{fig:chatCompletion} being model and messages. The model specifies which OpenAI model should be used to answer the request. Messages must be an array of message objects, where each object has a role, either "system", "user", or "assistant" and content. A conversation is formatted with a "system" message first, followed by alternating "user" and "assistant" messages. The "system" message is used to set the behavior of the assistant throughout the conversation. The "user" message provides requests or comments for the assistant to respond to. The "assistant" message can be either previous responses or examples of desired behavior. The full conversation history must be provided when user instructions refer to prior messages. If a conversation can not fit within the model’s token limit, it needs to be shortened.
A chat completion response is presented in Figure~\ref{fig:chatCompletionResponse}. The message generated by the model can be accessed by going through the attributes in the following order "choices", array index 0, "message", and "content". %Another relevant attribute is finish\_reason which can have the values of "stop" if successful, "length" if the token limit was reached, "function\_call" if the model called a function, "content\_filter" if some content was omitted, or "null" if response is still in progress. 
All the other values provide contextual information about the generated response~\cite{ref:openAI}. 
\begin{figure}[h]
    \lstinputlisting[style=json]{./code/chatCompletionResponse.json}
    \caption[Chat completion response]{Chat completion response~\cite{ref:openAI}%~\footref{foot:chatCompletion}
    }
    \label{fig:chatCompletionResponse}
\end{figure}

The LLMs are also capable of preparing an interaction with external tools through the use of the function calling~\hyperfootnote{https://platform.openai.com/docs/guides/function-calling}{foot:functionCalling} capability. To use this feature, the functions must be described in the tools~\hyperfootnote{https://platform.openai.com/docs/api-reference/chat/create}{foot:apiReference} attribute of the request, and then the model will generate an output that contains arguments to call one or more functions, see Figure~\ref{fig:functionCalling} for an example. A great advantage of function calling is that it allows to reliably get structured data from the model. Function calling can be used, for example, by assistants to call external APIs or to convert natural language into API calls~\cite{ref:openAI}.
\begin{figure}[h]
    \lstinputlisting[style=python]{./code/functionCalling.py}
    \caption[Function calling]{Function calling}
    \label{fig:functionCalling}
\end{figure}

An Assistant\hyperfootnote{https://platform.openai.com/docs/assistants/overview}{foot:assistant} is created with instructions that can leverage models, tools, and knowledge to respond to user queries. When creating an assistant, the developer can specify several parameters to configure it. Instructions are used to tell how the assistant should behave or respond. The model parameter specifies which GPT model the assistant will use. Tools built and supported by OpenAI can also be specified. Currently, there are three available tool types: code interpreter, retrieval, and function calling. The function's parameter allows the definition of custom function signatures to be used by the assistant. To use an assistant, a user should create a thread at the beginning of the conversation. Each thread should be related to a distinct conversation. This implies that the assistant is capable of handling multiple threads at the same time. The assistant ensures that the request will fit within the model's maximum context window. After creating a thread, a user can pass all the user-specific context information and files by creating a message. For the assistant to respond to the user's messages, a run must be created. This makes the assistant read the thread and decide the best way to answer the query. As the run progresses the assistant appends messages to the thread with its respective role. When the run reaches the completed status it is possible to list all the messages in the thread~\cite{ref:openAI}.

OpenAI has also made available prompt strategies\hyperfootnote{https://platform.openai.com/docs/guides/prompt-engineering}{foot:promptStrategies} to get better results and some prompt examples\hyperfootnote{https://platform.openai.com/examples}{foot:promptExamples} to showcase the model's capabilities. If prompt optimization is not enough to get acceptable results OpenAI provides a detailed guide on how to fine-tune a model\hyperfootnote{https://platform.openai.com/docs/guides/fine-tuning}{foot:fineTuning} using its API. Additionally, OpenAI Cookbook\hyperfootnote{https://cookbook.openai.com/}{foot:cookbook} provides access to more in-depth examples, use cases, and code snippets of common tasks~\cite{ref:openAI}.

%\subsection{GitHub Copilot}
%- What is Copilot?
%- What does it offer us?

%\subsection{LLM for test generation}
%- Use cases of LLM in test generation

\section{Web APIs} \label{sec:API}

% TODO Falar do uso de APIS e dimensão das mesmas

%What is an API?
At its basis, APIs are mechanisms that enable two software components to communicate with each other using a set of definitions and protocols. API stands for Application Programming Interface. The word application refers to any software with a distinct function. Interface can be thought of as a contract of service between two applications. This contract defines how two applications programmatically communicate with each other, using requests and responses~\cite{ref:apiAWS}.%~\hyperfootnote{https://aws.amazon.com/what-is/api/}{foot:apiAWS}. 

%APIs Integration
An API architecture is usually composed of a client and a server. The application sending the request is called the client, and the application sending the response is called the server. Resources are the information that the server provides to the clients~\cite{ref:apiAWS}. %~\footref{foot:apiAWS}. 
API servers act as a mediator between clients and the resources they want to get~\cite{ref:restRedHat}. %~\hyperfootnote{https://www.redhat.com/en/topics/api/what-is-a-rest-api}{foot:restRedHat}. 
One of the key properties of APIs is that they can be integrated into various software components, allowing them to update data automatically. Companies can also use APIs to automate multiple system functions efficiently. There are four main API architectures for distributed systems:
\begin{itemize}
    \item SOAP APIs: These APIs use Simple Object Access Protocol. Client and server exchange messages using XML. This less flexible API was more popular in the past~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.    
    \item RPC APIs: These APIs are called Remote Procedure Calls. The client calls a remote procedure on the server, and the server sends the output back to the client~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.
    \item Websocket APIs: These API uses JavaScript Object Notation (JSON) objects to pass data. It supports two-way communication between the client application and the server. The server can send callback messages to connected clients, making it more efficient~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.
    \item REST APIs: These are the most popular and flexible APIs found on the web today. The client sends requests to the server as data. The server uses this client input to start internal functions and returns output data to the client~\cite{ref:apiAWS}. %~\footref{foot:apiAWS}. 
    In this project, we will look at REST APIs in more detail.
\end{itemize}

APIs can also be classified according to their scope of use~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}:
\begin{itemize}
    \item Private APIs: These are internal to a company and are only used for connecting systems and data within the business.
    \item Public APIs: These are open to the public and may be used by anyone. There may or may not be some authorization and cost associated with these types of APIs.
    \item Partner APIs: These are only accessible by authorized external developers to aid in partnerships.
    \item Composite APIs: These combine two or more different APIs to address complex system requirements or behaviors. 
\end{itemize}

%API endpoints are an integral part of the API communication system that facilitates their integration. Endpoints are critical components due to security and performance reasons. Security-wise, they are the door for the application resources, making them vulnerable to attacks. Performance-wise, endpoints with high traffic can cause bottlenecks and affect system performance. Monitoring and testing are crucial to prevent these issues~\cite{ref:apiAWS}.

%What is a RESTful API? 
\subsection{RESTful API}

A RESTful API is an interface that two computer systems use to exchange information over the internet. Their wide adoption is mainly due to the secure, reliable, and efficient software communication standards that it follows, the REST architectural style~\cite{ref:restRedHat}. %~\footref{foot:restRedHat}. 
APIs that follow the REST style are called REST APIs. Examples of REST APIs are, for example, database services where you place your query and get back results. Web services that implement REST architecture are called RESTful web services. The term RESTful API generally refers to REST web services where you request data~\cite{ref:restAWS}.%~\hyperfootnote{https://aws.amazon.com/what-is/restful-api/}{foot:restAWS}.

REST stands for Representational State Transfer, and it imposes conditions on how an API should work. The principles of the REST architecture style are the following:
\begin{itemize}
    \item HTTP requests: client-server architecture made up of clients, servers, and resources, with requests managed through Hypertext Transfer Protocol (HTTP)~\cite{ref:restRedHat}.%~\footref{foot:restRedHat}. 
    \item Uniform interface: Indicates that the server transfers information in a standard format. The formatted resource is called a representation~\cite{ref:restAWS}.%~\footref{foot:restAWS}.
    \item Statelessness: The Server completes every client request independently of all previous requests. Clients can request resources in any order, and every request is stateless or isolated from other requests~\cite{ref:restAWS}.%~\footref{foot:restAWS}. %This REST API design constraint implies that the server can completely understand and fulfill the request every time.
    \item Layered system: Organizes each type of server involved in the retrieval of requested information into hierarchies, invisible to the client~\cite{ref:restRedHat}.%~\footref{foot:restRedHat}.
    \item Cacheability: Process of storing some responses on the client or on an intermediary to improve server response time~\cite{ref:restAWS}.%~\footref{foot:restAWS}.
    \item Code on demand: Servers can temporarily extend or customize client functionality by transferring software programming code to the client~\cite{ref:restAWS}.%~\footref{foot:restAWS}. 
\end{itemize}

%Request structure
The main components of an HTTP request and response are the following:
\begin{itemize}
    \item Unique resource identifier: In REST API, the server typically performs resource identification using a Uniform Resource Locator (URL). The URL specifies the path to the resource. The URL is a request endpoint that identifies the client's requirements for the server~\cite{ref:restAWS}.%~\footref{foot:restAWS}.
    \item Method: An HTTP method tells the server what action needs to be done to the resource. The most common methods are GET, POST, PUT, and DELETE.
    \item Headers: Store the metadata exchanged between the client and server. For example, the request header \textit{Content-Type} indicates the request and response format.
    \item Body: Includes extra information required for the method to work successfully. 
    \item Status Code: A numerical value composed of 3 digits that the server uses to tell the request's result.
\end{itemize}

%REST defines a set of functions like GET, POST, PUT, and DELETE. that clients can use to access server data. Clients and servers exchange data using HTTP~\cite{ref:apiAWS}.

%Rest benefits
The extensive adoption of RESTful APIs can be attributed to various factors. A few of the benefits include the following:
\begin{itemize}
    \item Integration: Allow the integration of new applications with existing software systems. This increases development speed because each functionality does not have to be written from scratch~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.
    \item Innovation: New applications can arrive at any time. Companies need to respond quickly to change and support the rapid deployment of innovative services. They can do this by making changes at the API level without having to rewrite the whole code~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.
    \item Flexibility: Support total client-server separation. REST APIs simplify and decouple various server components so that each part can evolve independently~\cite{ref:restAWS}.%~\footref{foot:restAWS}.
    \item Expansion: Offers the opportunity to meet clients' needs across different platforms. Any company can give access to its internal resources by using an API~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.
    \item Ease of maintenance: The API is a gateway between two systems. Each system is obliged to make internal changes so that the API is not impacted. This way, any future code changes by one party do not affect the other party~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}.
\end{itemize}

REST APIs are secured through authentication methods to prevent a service's misuse. 
Authentication tokens are used to authorize users to call the API. This mechanism checks the user's identity and access rights for the particular resources through its token. 
API keys verify the program or application making the API call. The server assigns a unique generated value to a first-time client. Whenever the client tries to access resources, it uses the unique API key to verify itself. API keys are considered less secure. 
OAuth combines passwords and tokens for highly secure login access to any system. The server first requests a password and then asks for an additional token to complete the authorization process. The token can be checked at any time and over time with a specific scope and longevity~\cite{ref:restAWS}.%~\footref{foot:restAWS}.

 %Rest secure
\subsection{OpenAPI Specification}

All modern software makes heavy use of APIs. Therefore, learning to use new APIs is an everyday task many developers face. To assist in this task, APIs are typically deployed with documentation~\cite{ref:apiDocumentation}. Being capable of providing good API documentation can determine its adoption success.
This documentation contains information on how developers should use the API. Typically, they have simple explanations written in a beginner's style. They can also include some code samples to help explain some functionalities. Recurrent maintenance is expected to keep it accurate and up-to-date. Standard specifications format, such as OpenAPI Specification (OAS), should be followed to keep the documentation process repeatable, concise, and deterministic.

The OAS provides consistent means to carry information through each stage of the API lifecycle. See Figure~\ref{fig:apiLifecycle}.
\begin{figure}[h]
    \includegraphics[width=0.45\textwidth]{figures/apiLifecyle.pdf}
    \caption[API Lifecycle]{API Lifecycle~\cite{ref:openAPI}%~\footref{foot:openAPI}
    }
    \label{fig:apiLifecycle} 
\end{figure}
OAS specifies an API structure and syntax independent from the programming language where the API was created. It is typically written in Yet Another Markup Language (YAML) or JSON, making it easy to share and consult. It also provides a comprehensive dictionary of terms that reflect commonly understood concepts in the world of APIs. OAS is an excellent way for developers to discover how an API works and understand system capabilities~\cite{ref:openAPI}.%~\hyperfootnote{https://www.openapis.org/what-is-openapi}{foot:openAPI}. %For more advanced users, it also allows them to configure infrastructure, generate client code, and create test cases. 

In the requirements phase of the API lifecycle, see Figure~\ref{fig:apiLifecycle}, OAS helps to elicit the project requirements. At this stage, an initial OAS sketch allows the shaping of the initial ideas, making them easier to share. 
In the design phase, having OAS for consumption by others is vitally important, as it is the source of truth that groups all the requirements. 
With the finished design, developers can start working with the OpenAPI document to bring the application to life. 
OAS is also critical when configuring the API infrastructure to protect from malicious intents. The majority of API management tools allow the usage of  OpenAPI documents to generate configurations.
In the development phase, having the means to communicate with developers accelerates the process of exchanging information. Multiple tools like Swagger use OAS documents to provide a richer developer experience.
Testing APIs requires the same insights as consuming APIs since it is required to understand their structure, parameters, requests, and response definitions. Having an OpenAPI document explains what an API offers, allowing both humans and computers to understand the capabilities of the service~\cite{ref:openApiSpecification}. 

As described before, OAS presents a straightforward structure, and some of the most relevant components are highlighted in this section.

OpenAPI object is the root object of the OpenAPI document. It consists of a version number of the OAS that the document uses~\cite{ref:openApiSpecification}. %~\hyperfootnote{https://swagger.io/specification/}{foot:openAPISpecification}
See Figure~\ref{fig:openApiObject}.
\begin{figure}[h]
    \begin{lstlisting}[style=yaml]
    openapi: 3.0.3
    \end{lstlisting}
    \caption[Example of OpenAPI Object]{Example of OpenAPI Object~\cite{ref:openApiSpecification}%~\footref{foot:openAPISpecification}
    }
    \label{fig:openApiObject} 
\end{figure}

An info object provides metadata about the API. The metadata may be used by the clients if needed and presented by documentation tools as convenient. See Figure~\ref{fig:infoObject}.
\begin{figure}[h]
    \begin{lstlisting}[style=yaml]
    title: Sample Pet Store App
    summary: A pet store manager.
    description: This is a sample server for a pet store.
    termsOfService: https://example.com/terms/
    contact:
      name: API Support
      url: https://www.example.com/support
      email: support@example.com
    license:
      name: Apache 2.0
      url: https://www.apache.org/licenses/LICENSE-2.0.html
    version: 1.0.1
    \end{lstlisting}
    \caption[Example of Info Object]{Example of Info Object~\cite{ref:openApiSpecification}%~\footref{foot:openAPISpecification}
    }
    \label{fig:infoObject} 
\end{figure}

A server object represents a server. It is composed of a URL to the target host. It may also include a small description that provides some more details. See Figure~\ref{fig:serverObject}.
\begin{figure}[h]
    \begin{lstlisting}[style=yaml]
    url: https://development.gigantic-server.com/v1
    description: Development server
    \end{lstlisting}
    \caption[Example of Server Object]{Example of Server Object~\cite{ref:openApiSpecification}%~\footref{foot:openAPISpecification}
    }
    \label{fig:serverObject} 
\end{figure}

A paths object holds the relative paths to the individual endpoints and their operations. The path is appended to the URL from the server object to construct the request's full URL. Some relevant fields to consider are the operation field specifying which HTTP operation this request does. It also includes a list of all possible response outcomes when executing the operation. See Figure~\ref{fig:pathsObject}.
\begin{figure}[h!]
    \begin{lstlisting}[style=yaml]
    /pets:
      get:
        description: Returns all pets from the system that the user has access to
        responses:
          '200':
            description: A list of pets.
            content:
              application/json:
                schema:
                  type: array
                  items:
                    $ref: '#/components/schemas/pet'
    \end{lstlisting}
    \caption[Example of Paths Object]{Example of Paths Object~\cite{ref:openApiSpecification}%~\footref{foot:openAPISpecification}
    }
    \label{fig:pathsObject} 
\end{figure}

\subsection{Swagger}

Supporting tools can provide a rich experience based on a simple document. Swagger, for instance, can parse OAS files and automatically build beautiful and interactive API documentation~\cite{ref:swagger}. %~\hyperfootnote{https://swagger.io/docs/specification/2-0/what-is-swagger/}{foot:swagger}. 
The swagger editor is an excellent tool for this purpose, see Figure~\ref{fig:swagger}.

\begin{figure}[h!]
    \includegraphics[width=0.6\textwidth]{figures/swagger.pdf}
    \caption[Swagger Editor]{Swagger Editor~\cite{ref:swaggerEditor}}
    \label{fig:swagger} 
\end{figure}

Despite the importance of API documentation, the study of Michael Meng suggests that developers, when learning how to use a new API, prefer to use search engines to locate information instead of querying the documentation offered by the API supplier~\cite{ref:apiDocumentation}. %page.32

\subsection{API Testing}

When an API provider puts their applications on the market, they need assurance that their APIs meet acceptable levels of quality and accuracy. Passing the API through a series of tests is a way to guarantee these requirements. Additionally, any unprecedented change in the APIs can cause a significant failure of service operations, which can cause the provider to face major losses~\cite{ref:APITestMethods}.

API testing strategies are similar to other software testing methodologies. The main focus is on validating server responses. API testing includes making multiple requests to API endpoints to test their performance, writing unit tests to check business logic and functional correctness, or even performing security tests by simulating system attacks~\cite{ref:apiAWS}.%~\footref{foot:apiAWS}. 

%Test automation
There are different testing levels, depending on the nature of the element being tested, but not all should be automated. Unitary-level tests focus on testing small software units, the integration-testing level focuses on the interaction between units, and the system-testing level focuses on complete functionalities~\cite{ref:testAutomation}. These test types are normally described as functional tests, which aim to verify whether the product does what it should.

Test automation is the practice of generating and running tests automatically, managing test data, and recording results to improve software quality. Testing is primarily a quality assurance measure, but its activities involve the commitment of the entire software production team. From business analysts to developers and DevOps engineers, getting the most out of test automation takes the inclusion of everyone~\cite{ref:whatIsTestAutomation}.%~\hyperfootnote{https://www.testim.io/blog/what-is-test-automation/}{foot:whatIsTestAutomation}.

One primary goal of automated testing is to save time, effort, and money. Some studies suggest that testing consumes 30 to 60 percent of all the product life-cycle costs~\cite{ref:testAutomation}. To be automated, a test needs to meet some criteria. Otherwise, it may cost more than it saves. A test must be repeatable, allowing it to be executed multiple times, determinant, since the outcome must be the same every time it is run with the same input, and unopinionated, since the test result should not be dependent on human opinions~\cite{ref:whatIsTestAutomation}.%~\footref{foot:whatIsTestAutomation}.

There are three essential stages when performing automated testing: preparing, executing, and reporting.
\begin{itemize}
    \item \textbf{Preparing}: The first step where the application state, the test data, and the environment where tests will be executed should be prepared. The environment must be in the required state before any test execution. This implies that either the application data needs to be manipulated or the application needs to be placed into a specific state.
    \item \textbf{Executing}: After the state and environment are set up, the tests can be executed. The selected testing platform should run the test previously created either by calling an application's API or by directly running the code. The testing platform is responsible for coordinating everything. This includes controlling the execution of the test cases and reporting the test results.
    \item \textbf{Reporting}: Lastly, the reported results must be analyzed. A test's result is expected to be either a pass or a fail. However, these results may come in several formats and generate new issues or bugs in the project tracking system. Sometimes, tests are inconclusive or don't run for some reason. When this happens, the automation system should create a complete output log for developers to review. This log helps them track down the issue~\cite{ref:whatIsTestAutomation}.
\end{itemize}

%API test types
In recent years, multiple research efforts have been made to alleviate RESTful API testing challenges by introducing different frameworks and auto-generating unit test approaches. Unit tests focus on confirming that a single endpoint returns the correct response to a given request. Due to the lack of more autonomous and comprehensive technologies, these auto-generating methods mainly focus on achieving a high line execution code coverage~\cite{ref:APITestMethods}. This metric can be misleading as it may not test the system's unique properties since coverage only validates the execution of a given part of the code but the paths taken before and after the line execution. 
End-to-end or integration testing is another test type that validates user journeys involving multiple API endpoints. These tests include chaining requests together and confirming that each one is working correctly. This helps teams discover issues in complex workflows~\cite{ref:postmanApiTest}. %~\hyperfootnote{https://www.postman.com/api-platform/api-testing/}{foot:postmanApiTest}. 
Since end-to-end tests focus on validating the application's business logic, they require more comprehension of the systems, which makes them more complex to create. 
Techniques to test non-ordinary inputs are also presented in the literature. Fuzz testing involves feeding unexpected and invalid inputs into the API to test its ability to handle unexpected inputs and recover from errors. This type of testing can uncover security vulnerabilities or unexpected behavior in the API~\cite{ref:impervaApiTest}. %~\hyperfootnote{https://www.imperva.com/learn/application-security/api-testing/}{foot:impervaApiTest}.

Normally, different test types require distinct modules. These modules are composed of oracles. An oracle is a function that tells whether a test was successful. To better understand the need for oracles, let us consider manual testing, where the developers need to decide what the expected result should be for a given test case and write such expectation as an assertion check directly in the test cases. In automated test generation, where many hundreds if not thousands of test cases are generated, asking the developers to write such assertions is not a viable option~\cite{ref:apiAutomatedTestGeneration}. 

For example, the RESTTESTGEN tool~\cite{ref:apiBlackBoxTesting} uses two distinct oracles, which are the following: 
\begin{enumerate}
    \item A \textbf{status code oracle} that analyses the three digit integer value in the HTTP response meant to describe the outcome of a request. A status code in the form 2xx stands for a correct execution. A status code 4xx stands for an error that was correctly handled. Conversely, a status code 5xx means that the server encountered an error that was not handled correctly. 
    \item A \textbf{response validation oracle} that checks for mismatches between the intended response syntax, documented in the Swagger, and the actual response, observed at execution time, by using a schema validation library~\cite{ref:apiBlackBoxTesting}. 
\end{enumerate}
The RESTTESTGEN solution is very similar to ours as it aims to test APIs from two perspectives. Nominal execution scenarios test the system using input data as it is documented in the interface, while error execution scenarios exploit input data that violate the interface to expose implementation defects and unhandled exceptional flows. RESTTESTGEN uses an operation dependency graph to guess whether a new operation can be tested.

Another simpler example is Laura Plein's solution~\cite{ref:testCasesFromBugReport}, where she directly prompts ChatGPT with a prompt that concatenates the instruction, as follows \textit{“write a Java test case for the following bug report: ...”}, and the bug report. The informal bug reports are written by application users. This white-box approach differs from our proposed solution since, firstly, we will not have access to the application's source code, and secondly, we expect to use test scenarios described more formally. Nevertheless, the work developed provides excellent insights into what we can expect, as it shows the capabilities of LLMs to generate test code.

Lastly, another white-box approach is EvoMaster~\cite{ref:apiAutomatedTestGeneration}, which automatically generates integration tests for API services. The technique aims to maximize code coverage and find faults using the HTTP return statuses as an automated oracle.
To generate the tests, they employed an evolutionary algorithm, particularly a Genetic Algorithm. Similar to our approach, it requires the openAPI specification. However, they require access to the application source code to measure statement coverage. This differs from our solution as we will measure coverage based on the available API services.

A great way to effectively perform API testing involves using platforms that provide automated processes. Insomnia~\cite{ref:insomnia} %~\hyperfootnote{https://insomnia.rest/}{foot:insomnia} 
and Postman~\cite{ref:postman} 
%~\hyperfootnote{https://www.postman.com/}{foot:postman} 
are two platforms that serve these purposes and are widely used in the software industry. Both provide functionalities related to API design, debugging, and testing. Regarding the testing, these platforms allow the automation of the test execution during the entire API lifecycle. The main difference is the pricing model that each of them uses. Insomnia is an open-source tool that is free to use, while Postman requires the payment of a monthly fee. Traditional programming languages, such as python, javascript, java, typescript and more, are also commonly used to build tests for API services~\cite{ref:apiAutomatedTestGeneration}~\cite{ref:restApiFuzzing}~\cite{ref:apiBlackBoxTesting}~\cite{ref:testCasesFromBugReport}.

\section{Summary} \label{sec:summary}

The chapter offers an overview of key concepts and practices relevant to the project, focusing on generative AI, Web APIs, and test automation.

Generative AI and LLMs are central to the discussion. Generative AI refers to models capable of generating content such as text, code, images, videos, and music. These models are distinguished by their ability to create complex outputs dynamically. LLMs, a subset of generative AI, are specifically trained to perform various natural language processing tasks. 

The use cases of LLMs are diverse, including information retrieval, code generation, conversational AI, and creative work. They are used in fields such as technology and management, highlighting their broad applicability. The benefits of LLMs include their ability to improve over time with more data, their scalability, and their capacity to provide users with a wide range of skills. However, challenges such as hallucinations, prompt brittleness, security risks, bias, consent issues, deployment complexities, outdated knowledge, and tasks not solvable by scale persist.

Prompt engineering, a critical aspect of using LLMs, involves designing queries to achieve desired outputs. Techniques in prompt engineering include RAG, chain-of-thought, and tree-of-thought. Evaluation metrics can be used to measure LLM performance. Popular LLM tools discussed include GPT-4, GPT-3.5, Gemini Pro, Claude 2, and LLAMA 2, each with specific strengths and applications. Additionally, tools for code generation and suggestion built on top of LLMs, such as GitHub Copilot and Amazon CodeWhisperer, are highlighted for their ability to enhance developer productivity.

Web APIs are another focus area. APIs enable software components to communicate using requests and responses. They use HTTP methods and include components such as unique resource identifiers, headers, and status codes. API documentation is essential for understanding and using APIs, often written in OAS format. The OAS provides a consistent structure for documenting APIs throughout their lifecycle. Tools like Swagger parse OAS files to build interactive API documentation. API testing ensures that APIs meet quality standards through various methods, including unit tests, integration tests, and fuzz testing.

Testing automation is the practice of generating and running tests automatically, managing test data, and recording results to improve software quality. It involves preparing the environment and data, executing tests, and reporting results. Automated tests must be repeatable and deterministic.

Overall, the chapter provides a detailed foundation on generative AI, APIs, and test automation, emphasizing their relevance, benefits, challenges, and methodologies in a software development context.

In this thesis, we explore various available LLMs and prompt engineering techniques to create an API test automation tool and compare it with existing tools.

==> Tese_Andre/chapter3.tex <==
\chapter{APITestGenie} \label{chap:solut}

This chapter introduces APITestGenie, an innovative tool designed to assist users in autonomously creating API tests with ease and efficiency. The tool is envisioned to meet Critical Techwork's needs. Therefore, we have iteratively improved our approach according to the requirements and feedback that we received. Section~\ref{sec:data} describes the data used throughout the project and its manipulation. Section~\ref{sec:technologies} highlights the key technologies, tools, and frameworks employed. The architecture of the autonomous test generation tool is detailed in Section~\ref{sec:architecture}. Section~\ref{sec:promptEngineering} explores the key prompt engineering techniques used during project development and some recommendations. Finally, Section~\ref{sec:solutionWorkflow} presents a prototype showcasing how the solution could be used. 

\section{Data} \label{sec:data}

In such a data-dependent application, having the right data is crucial. According to our needs, preliminary work to collect all the required data was put in place. This involved creating various pipelines to automate the processes of collecting, cleaning, and filtering relevant data, with the goal of developing a fully autonomous tool. The collected data includes business requirements from user stories and sequence diagrams, as well as OpenAPI specifications from different services.

Business requirement describes a use case to be tested. The level of detail of the business requirement may vary, resulting in different outcomes when using the tool. The various detail levels used in the solution will be further explored in Section~\ref{sec:promptEngineering}. Business requirements were retrieved from user stories documented in project management tools and sequence diagrams provided by the development team in the technical documentation of the project. The selection criteria involved relevance to the project scope, if the business requirement is related to the API and completeness of the information.

User stories are a valuable source for collecting business requirements, as their purpose is to explain an expected software feature. In addition to the title and description, some user stories are accompanied by more information like acceptance criteria, development hints, inputs, expected results, and additional information. This provided us with a more comprehensive context of business requirements, which proved advantageous. Although sequence diagrams were not directly used as inputs in our system, they proved valuable for mapping the interactions among multiple services. By analyzing and summarizing these interactions, we identified various use cases. This enabled us to generate unique natural language prompts that described business requirements, which we could then use as input.

OpenAPI specifications play a critical role in our solution, so various APIs with different characteristics were collected. This allowed us to validate the solution in different environments and under different constraints. Table~\ref{tab:apiSpecification} lists all the API specifications used in the project. The number of tokens was calculated using the tiktoken tokenizer~\cite{ref:tiktoken} that turns text into tokens. We used \textit{cl100k\_base}~\cite{ref:howToTokenize} encoding format, which most GPT models use to process text inputs. The \textit{Original Tokens} was calculated using the original API specification document. While the \textit{Simplified Tokens} was calculated using the simplified API specification. The pre-processing tasks performed on the original API specification that led to the simplified API specification are explained later in this Section. The access describes whether the API documentation is publicly available or maintained by the company and, therefore, private. Public available APIs can be accessed in CatFact~\hyperfootnote{https://catfact.ninja/}{foot:catFact} and PetShop~\hyperfootnote{https://petstore.swagger.io/}{foot:petShop}. Private APIs contain sensitive Critical Techworks data that provide access to information about their clients and products. Furthermore, the private APIs under test are highly used in BMW applications, and their integrity is required to maintain the application's correct functioning. Due to confidentiality reasons, we can not describe them further.

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c|c|c}
         \textbf{Service} & \textbf{Original Tokens} & \textbf{Simplified Tokens} & \textbf{Access} \\ \hline
         Cat Fact & 754 & 754 & Public \\
         Pet Shop & 4,070 & 4,070 & Public \\
         GCDM Customer & 25,966 & 25,473 & Private \\
         GCDM & 47,497 & 47,004 & Private \\
         OneShop & 49,761 & 49,761 & Private \\
         UCP Accessories & 882,272 & 14,018 & Private \\
         UCP Otd & 430,739 & 16,094 & Private \\
         UCP Localisations & 1,620,488 & 82,267 & Private \\
         UCP Vehicles & 417,109 & 108,724 & Private \\
         UCP All & 5,021,555 & 424,465 & Private \\
    \end{tabular}
    \caption[List of API specifications used in this project.]{List of API specifications used in this project. Describes the API's original and simplified number of tokens and type of access.}
    \label{tab:apiSpecification}
\end{table}

Figure~\ref{fig:APIMatrix} provides an overview of the characteristics of the API services used in the project. We evaluated the APIs in two dimensions visible in the matrix: complexity/restrictions and documentation detail. The horizontal axis evaluates if a given API specification thoroughly explains each available resource, containing usage examples and all the possible outcomes. The vertical axis evaluates the complexity and restrictions of the API. It is mainly related to security constraints and how information needed to perform the test can be collected. Each quadrant is associated with a suggested prompt level that we detail in Section~\ref{sec:promptEngineering}. \textit{Cat Fact}, \textit{Pet Shop}, and \textit{UCP Otd} are both in the green area of the matrix, meaning that the service is easy to interpret with the available documentation. \textit{UCP Localization}, \textit{UCP Accessories}, \textit{UCP Vechicles}, \textit{GCDM Customer}, and \textit{GCDM} are all in the yellow area, meaning that, after reading the documentation and doing some experiments, it is possible to get a grasp of the functioning of the API.  \textit{UCP All} is an exceptional case from the yellow area. Due to its high complexity and API dimension, it requires a prompt level 3. \textit{OneShop} requires the user to know the system business logic to use the API and be able to generate tests for the API. This API characterization is highly related to the suggested business requirement level of detail, explained in more detail in Section~\ref{sec:promptEngineering}.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/APIMatrixPrompt.pdf}
    \caption[API characterization matrix.]{API characterization matrix. Evaluates the different APIs based on their internal complexity and the level of detail of the specification. Associates each matrix quadrant to a specific prompt level.}
    \label{fig:APIMatrix}
\end{figure}

To effectively use the API specifications, an initial pre-processing was performed to remove irrelevant and unused information. At first, data processing was performed manually to understand the specific requirements and nuances of different APIs, allowing us to filter and select the information that could be relevant to the test generation process. However, as the number and size of APIs increased, this manual approach did not scale. We developed a more general approach by leveraging the knowledge gained from the manual process. The approach resulted in a script that removed all the \textit{<img>} tags and all the \textit{admin} and \textit{deprecated} resources in the API specification. These optimizations were more effective in the UCP APIs due to large SVG images present in their specification that were irrelevant to our use case. \textit{UCP Localisations} is the API with the most notorious optimization, since before the pre-processing, it had 1,620,488 tokens, and after 82,267 tokens, reducing its size by almost twenty times.

\section{Technologies} \label{sec:technologies}

The core component of our project is the LLM. Its access can be made in multiple ways, either through a user interface or via an API. Since we wanted to develop a fully autonomous tool, using an API to interact with the LLM was mandatory. Initially, we started by running the smaller model of LLAMA2 7B locally. However, the generation proved to be very slow, and the outputs did not meet our expectations in terms of quality. In the experiment presented in Figure~\ref{fig:llama2Prompt}, the generated response is clearly not the expected result given the provided prompt. With this run, we expected a small code script that can be executed. However, it generated a random comment that related to our topic. Appendix~\ref{apx:gptSortArray} shows a generation done using GPT-4 LLM with the same prompt that meets our expectations. This experiment highlights that to evaluate the real capabilities of this generative AI, we need to execute and use the larger and more capable LLMs.

\begin{figure}[h]
    \begin{lstlisting}[style=prompt_history]
Prompt: Generete a valid Typescript test using Jest and axios library to sort a list of integers
Response: Comment: @T.J.Crowder I'm not sure what you mean. I'm trying to return the sorted list of integers.
    \end{lstlisting}
    \caption[LlamaCode-2-7b-instruct sorted array test generation]{LlamaCode-2-7b-instruct sorted array test generation in 197 seconds. Model executed locally in a windows machine with i7-12800H and NVIDIA GeForce RTX 3050 Ti.}
    \label{fig:llama2Prompt} 
\end{figure}

With the type of LLMs we wanted to use selected, we now need to choose a cloud provider that makes them available. Our choice was influenced by two main criteria: guaranteeing the data privacy constraints of the company and ensuring the availability of the models that we wanted to test, LLAMA and GPT. Azure ended up being the cloud provider that best fits our needs. It made available multiple LLM versions of GPT and LLAMA that we could test while guaranteeing all the data constraints that we had. There were two Azure services that we made use of:
\begin{enumerate}
    \item \textbf{Azure OpenAI Studio}: Used to access openAI resources, GPT-4, GPT-4-Turbo, GPT-3.5-Turbo, and ada embedding model through a secure and scalable API.
    \item \textbf{Azure Machine Learning Studio}: Used to access open source models, like LLAMA, through on-demand APIs or by hosting and deploying in a virtual machine. Additionally, provides access to prompt flow, a tool that helps develop AI-powered applications establishing the connection of LLMs and prompts. Prompt flow allowed the creation of different executable flows that we deployed in a real-time endpoint using \textit{Docker} containers~\cite{ref:docker}. These flows were designed to systematically query the LLM, ensuring that the generated responses were relevant and useful for our testing purposes.
\end{enumerate}
Both of these services provide a detailed cost analysis that is also relevant to our research.

The development of our solution relied heavily on Python for scripting, data processing, and integration with other tools and services. Python's versatility and extensive libraries made it an ideal choice for these projects. Some key libraries used include:

\begin{itemize}
    \item \textbf{LangChain}~\cite{ref:langChain}: Facilitated tasks to store, index, and retrieve data, such as OpenAPI specifications, and establish connections to LLMs.
    \item \textbf{ChromaDB}~\cite{ref:chroma}: A local database solution used for storing and retrieving embeddings efficiently, crucial for handling our data.
    \item \textbf{Tiktoken}~\cite{ref:tiktoken}: Utilized for tokenizing text inputs, it is useful to keep track of the input size constraints of LLMs.
    \item \textbf{get-code-from-markdown}~\cite{ref:getCodeFromMarkdown}: A utility to extract code snippets from markdown texts. Used to parse the generated test.
    \item \textbf{Streamlit}~\cite{ref:streamlit}: Used to create an interactive user interface for our tool, enabling real-time data visualization and interactions with the flows.
\end{itemize}

With the pipelines created, we started performing more complex runs with the models that we intended to use. Budget constraints were a deciding factor when selecting the primary model. We needed a real-time endpoint hosted in one of Azure's virtual machines to use a LLAMA model. The recommended machine, which would perform well, costs €10.35 per hour. Upon activating a machine, it will run for a complete hour. During the day, we need to test the code we developed, so the machine must be running. If we test our code in 3 distinct hours daily, the cost would be €31.05 per workday. This is a very high price to pay, given our budget. Therefore LLAMA models, \textit{CodeLlama-34b-Instruct-hf}~\hyperfootnote{https://ml.azure.com/models/CodeLlama-34b-Instruct-hf/version/9/catalog/registry/azureml-meta}{foot:codeLlama32bInstruct}, \textit{CodeLlama-34b-hf}~\hyperfootnote{https://ml.azure.com/models/CodeLlama-34b-hf/version/8/catalog/registry/azureml-meta}{foot:codeLlama32b}, \textit{CodeLlama-13b-hf}~\hyperfootnote{https://ml.azure.com/models/CodeLlama-13b-hf/version/9/catalog/registry/azureml-meta}{foot:codeLlama13b} and \textit{CodeLlama-13b-Instruct-hf}~\hyperfootnote{https://ml.azure.com/models/CodeLlama-13b-Instruct-hf/version/9/catalog/registry/azureml-meta}{foot:codeLlama13bInstruct} ended up being discarded.

On the other hand, GTP models are available via a pay-as-you-go pricing model that considers the number of input and output tokens to calculate the total amount to pay. Table~\ref{tab:gptPricing} provides an estimate of the expected costs using the LLMs from the GPT family.
\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
         \textbf{Model} & \textbf{Context}  & \textbf{Version}  & \textbf{Input} & \textbf{Output} & \textbf{Workday Estimate} \\ \hline
         GPT-3.5-Turbo & 16k & 1106 & €0.0010 & €0.0019 & €0.14 \\
         GPT-4 & 32k & 0613 & €0.056 & €0.111 & €7.72 \\
         GPT-4-Turbo & 128k & 1106-Preview & €0.010 & €0.028 & €1.42 \\
    \end{tabular}
    \caption[Pricing of GPT models.]{Pricing of GPT models. Input and output prices per 1000 tokens. Workday Estimate considers the input of 128k tokens and the output of 5k tokens.}
    \label{tab:gptPricing}
\end{table}
Considering the above analysis, the most cost-efficient model is GPT-4-Turbo. While GPT-3.5-Turbo is cheaper, its context size is too small for the data we aim to work with. According to Table~\ref{tab:apiSpecification}, only 3 out of 10 API specifications could be fully processed by the model. GPT-4 is significantly more expensive than GPT-4-Turbo, offering less performance and a smaller context size, leading to its immediate elimination. Also related to processing textual data, we used the \textit{text-embedding-ada-002}~\cite{ref:adaEmbedding} as our embedding model to create embeddings when needed.

Lastly, to validate the generated tests, we created a nodejs~\hyperfootnote{https://nodejs.org/en}{foot:node} environment capable of executing tests in TypeScript and collecting its results. The environment was set up with libraries such as Jest~\hyperfootnote{https://jestjs.io/}{foot:jest} to run the integration tests and Axios~\hyperfootnote{https://axios-http.com/docs/intro}{foot:axios} an HTTP client to make requests to the APIs. 

\section{Architecture}  \label{sec:architecture}

This section details the architecture of the proposed automated testing tool, which is capable of autonomously generating, refactoring, and executing test cases. The architecture is divided into three main flows: Test Generation, Test Refactoring, and Test Execution. Due to the modular approach, all three flows may be executed independently. However, they are expected to be used together, providing a more complete solution. See Figure~\ref{fig:architecture} for more detail. 

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{figures/architecture.pdf}
    \caption[Solution architecture.]{Solution architecture. Showcases the interactions of the three flows of the system: Test Generation, Test Refactoring, and Test Execution with the respective external inputs, tool outputs, external tools, and source of data either provided by the user in real-time or retrieved from a local or web file.}
    \label{fig:architecture}
\end{figure}

Each flow involves different processes, inputs, outputs, and tools, as follows:
\begin{itemize}
    \item \textbf{Test Generation Module} is the starting point of a new test generation.
        \begin{itemize}
            \item \textbf{Input}: Receives business requirements and API specifications described in Section~\ref{sec:data}.
            \item \textbf{Output}: Expected to generate an executable test script.
            \item \textbf{Tool}: Can use any LLM model with the correct setup.
        \end{itemize}
    \item \textbf{Test Execution Module} provides results of the generated test. It is expected to be the final point of the flow when the developer considers the generated test to be good.
        \begin{itemize}
            \item \textbf{Input}: Receives the script of the test generated by the Test Generation flow or the Test Refactoring flow.
            \item \textbf{Output}: Detailed report with the number of executed tests, failed tests, successful tests, and error messages.
            \item \textbf{Tool}: Can use the external Typescript environment to execute the tests.
        \end{itemize}
    \item \textbf{Test Refactoring Module} Generates a new test by iterating over the previous generations. It can be executed multiple times, given that a test script exists.
        \begin{itemize}
            \item \textbf{Input}: Receives the test generated by the Test Generation flow. If available, it can receive the Test Results, which allows it to improve the test if an error occurs. Optionally, the user can provide, on the fly, more context to get the desired results from the model.
            \item \textbf{Output}: Expected to generate an improved executable test script.
            \item \textbf{Tool}: Can use any LLM model with the correct setup.
        \end{itemize}
\end{itemize}

Each module is composed of smaller scripts with distinct tasks. This builds the flow's internal logic and allows us to easily update it with new or alternative functionalities. See Figures~\ref{fig:generation}, ~\ref{fig:execution}, and ~\ref{fig:refactoring} to get more details about the scripts used in the Test Generation, Test Execution, and Test Refactoring flows, respectively.

\subsection{Test Generation Module}

Figure~\ref{fig:generation} showcases the Test Generation flow internal logic. Due to the intrinsic creativity of the LLM, consecutive runs with the same data are expected to produce different results. The generation flow is our solution's entry point since it creates the first version of the test that we can use in the other two flows. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.6\linewidth]{figures/generationFlow.pdf}
    \caption[Generation Flow.]{Generation Flow. Showcases the flow of the data, starting from fetching the business requirement and API specification to the interaction with the Generative AI model.}
    \label{fig:generation}
\end{figure}

Following is a description of each script used in the flow:
\begin{itemize}
    \item \textbf{Fetch Business Requirement}: A seamless integration with the project management tool Jira is expected, so the user can provide the identifier of the project issue key, for example, \textit{SHOP-0000}. The script will then autonomously collect the relevant information, as described in Section~\ref{sec:data}. Alternatively, the user can provide a business requirement described in its own words. There are no constraints on its structure, so the tool can be used by distinct users as they see fit. Section~\ref{sec:promptEngineering} provides some guidelines for structuring the business requirement to get better results. 
    \item \textbf{Fetch API Specification}: Fetch API from a local file or web service. In this phase, the API specification pre-processing described in Section~\ref{sec:data} is performed. This reduces the size of data in use and accelerates the following processes.
    \item \textbf{Full API}: Forward the optimized API specification to the next steps. It executes exclusively from the RAG API script, explained in the next point. This means that only one of the scripts, either \textit{Full API} or \textit{RAG API}, is executed in a single flow execution.
    \item \textbf{RAG API}: Use RAG to retrieve the API specification chunks that are more similar to the business requirement, explained in more detail in Section~\ref{sec:promptEngineering}. This allows the LLM to retrieve relevant information from a large corpus, ensuring that the generated response is informed by the most pertinent context. This approach is expected to perform better when generating tests for APIs with larger contexts. RAG API can also be used to reduce the dimension of an API specification so that it can fit in the LLM context window, for instance, \textit{UCP All} API. Executes exclusively from Full API.
    \item \textbf{System Prompt}: Defines the main goal of the model by specifying the job he is expected to perform. When building the prompt, we followed the guidelines provided in TELeR taxonomy~\cite{ref:teler} of a Level 6 prompt. The system prompt presented in this section is the culmination of multiple iterations that allowed us to achieve the best performance. The system prompt can be divided into three main parts: Context, Performance, and Output Structure. See Figures~\ref{fig:systemPromptContext},~\ref{fig:systemPromptPerformance},~\ref{fig:systemPromptOutputStrucuture}, respectively. In the system prompt, we provide objective information and instructions that the LLM needs to follow and not reason about.

\begin{figure}[h!]
    \begin{lstlisting}[style=prompt]
As an AI coding assistant, my goal is to facilitate the creation of executable API integration tests in TypeScript.
Many users may not be familiar with coding, so I am here to bridge the gap and help them craft tests that validate their application's business requirements.

To ensure the tests are practical and meet the users' needs, I will generate integration test cases in TypeScript using the Axios and Jest libraries.
These tests will be designed for immediate execution and will interact with the API endpoints defined in the API specification.

I am expected to create more complex tests following the example:
***
{{test_example}}
***

When generating the test I will use existing environment variables. Following is the list of all available environment variables:
```
{{env_description}}
```
Each variable is denoted as `<environment name>:<description of the environment variable>`. I will load the variables that I need using the following code example:
`process.env.<environment name>`
    \end{lstlisting}
    \caption[System Prompt Context.]{System Prompt Context. Outlines the model persona as an AI coding assistant and provides guidelines the model should follow. It also specifies the high-level goal of the prompt. Additionally, the prompt includes an example test structure and information about available environment variables.}
    \label{fig:systemPromptContext}
\end{figure}
    
    The System Prompt Context, see Figure~\ref{fig:systemPromptContext}, specifies the main goal of the prompt, in this case, to generate integration tests for an API in TypeScript to validate a business requirement. It also describes the target user of the tool. To further refine the model output, in \textit{test\_example} placeholder, we provide a template of a typical test that we want the model to generate. Figure~\ref{fig:systemPromptTestExample} shows the test template that we use. Lastly, in the \textit{env\_description} placeholder, we list existing environment variables that the model can use in the requests. Since we are working with enterprise services, these variables are required as they provide secret keys to authenticate requests to access the resources. An entry of this list is composed of the environment variable name, followed by a description, for example: \textit{API\_SECRET\_KEY: "Secret key to authenticate the requests to cat facts API"}. This feature is crucial for security as it ensures that secret tokens remain confined to the execution environment. Another example of a variable that we have defined in this list is the request base endpoint path. Since the company uses multiple environments for testing its features, having the base path in an environment variable provides an easy way to switch between integration, production, test, and other environments.

\begin{figure}[h!]
    \begin{lstlisting}[style=python]
```typescript
import axios from 'axios';

 describe('General description of the test', () => {
   test('Specific description of the test', async () => {
     // Prepared test data
     data = {...}
     // Setup test environment
     // Make request with generated data
     const response = await axios.post(url, data);
     // Validate response of request
     expect(response...).toBe(...);
     // Add additional assertions based on response data                             
   });
   test('Another specific description of the test', async () => {                    
     // Prepared test data
     data = {...}
     // Setup test environment
     // Make request with generated data
     const response = await axios.get(url, data);
     // Validate response of request
     expect(response...).toBe(...);
     // Add additional assertions based on response data  
    });
    // Add more tests for other scenarios
    ...                                                                        
 });  
```
    \end{lstlisting}
    \caption[System Prompt TypeScript test example.]{System Prompt TypeScript test example. Expected structure of a TypeScript integration test generated by the model.}
    \label{fig:systemPromptTestExample} 
\end{figure}

\begin{figure}[h!]
    \begin{lstlisting}[style=prompt]
The tests will be assessed on several key factors:
**Executability**: The tests must run smoothly and without errors.
**Relevance**: The tests must be meaningful and appropriate for the requirement
**Correctness**: The test code should be free of logical errors.
**Coverage**: The tests should cover as many endpoints and scenarios as possible to ensure thorough validation.
**Code Quality**: The code is reliable, executable, and includes clear explanations where necessary.
**Endpoint Accuracy**: The API call matches the type of the request and response object. 

When generating tests, I will consider these important guidelines:
**Informational Completeness**: I will strive to collect as much information as possible. Additionally, I will generate experimental data to use in placeholders.
**Environment setup**: In the setup phase, I will make sure to collect all the data to guarantee that I have the data to execute the test.
    \end{lstlisting}
    \caption[System Prompt Performance.]{System Prompt Performance. Guidelines on how the LLM output will be evaluated.}
    \label{fig:systemPromptPerformance} 
\end{figure}

Following the System Prompt Performance, see Figure~\ref{fig:systemPromptPerformance}, which lists important guidelines describing how the model will be evaluated. Consistent with TELeR taxonomy conclusions~\cite{ref:teler}, we also found that rules phrased positively perform better than those that negate a behavior. This explains why the provided guidelines specify what is expected to be done rather than prohibiting certain behaviors. These guidelines were formulated after analyzing various runs, where we found recurrent and unwanted patterns. These instructions aim to restrict the model behavior, guiding the generated content towards the desired outcome.
\begin{figure}[h!]
    \begin{lstlisting}[style=prompt]
Here's how the test generation will be accomplished:

1. **Clarifying the Business Requirement**: In a summarized way, explain the business requirement, along with the specific aspects the tests are verifying.
I will describe the data and the environment state of the test.

2. **Listing Endpoints**: Then, I will list the endpoints that the test script will interact with. For each endpoint, I will specify the types of the request object and the types of the response object.
I will also provide a brief list of steps to reach the correct test environment state.

3. **Craft Executable Test Code**: Finally, I will generate code test cases in TypeScript using Axios and Jest libraries. The code must be presented in a single code block and ready to run. 
Make sure to explain any property that is unclear. Minimize any other prose.

Document your generation using the following format, and only provide information related to the generation step specified in the placeholder.
```
REQUIREMENT:
<1. **Clarifying the Business Requirement**>
ENDPOINTS:
<2. **Listing Endpoints**>
TEST:
"""typescript
<3. **Craft Executable Test Code**>
"""
```
    \end{lstlisting}
    \caption[System Prompt Output Structure.]{System Prompt Output Structure. Details expected output structure with a description of its components.}
    \label{fig:systemPromptOutputStrucuture} 
\end{figure}
Lastly, the System Prompt Output Structure, see Figure~\ref{fig:systemPromptOutputStrucuture} details how the model output should be formulated. The model must follow this structure since the following script, the parser, relies on the \textit{REQUIREMENT}, \textit{ENDPOINT}, and \textit{TEST} tags to collect the output. The \textit{REQUIREMENT} and \textit{ENDPOINT}, on top of providing the user with more context, are also used to guide the LLM reasoning process. These two initial steps allow the LLM to break the requirement into smaller tasks and list important information that will be necessary on the test script. With most of the reasoning done, when generating the \textit{TEST} tag, the model just needs to combine all the data to construct an executable test case. 

    \item \textbf{User Prompt}: Provides information specific to the business requirement that the model uses as content to generate the test script. The data provided in this prompt is expected to change in each execution according to the requirement under test.
\begin{figure}[h!]
\begin{lstlisting}[style=prompt]
Following is the business requirement that you will be testing.
This narrative will guide the creation of your tests and provide the context needed to determine the data for API requests.
Here is the business requirement for your reference:
***
{{user_story}}
***
Here are some instructions that may help you when generating the setup data for your tests:
***
{{setup_instructions}}
***
Next, you will review an API specification that details the available endpoints with the requests/response data structure.
The test you develop should validate the correct functioning of these endpoints
Ensure that you respect the requirements detailed in the specification and the request and response object types.
Here is the API specification:
***
{{api_specification}}
***
Let's start!
    \end{lstlisting}
    \caption[User Prompt Structure.]{User Prompt structure. Details of the prompt structure passed to the LLM, with placeholders for the business requirement and API specification.}
    \label{fig:userPrompt} 
\end{figure}
Figure~\ref{fig:userPrompt} showcases our latest User Prompt. The prompt starts by receiving the business requirement in the \textit{user\_story} placeholder. This information is provided at the beginning of the prompt, allowing the model to pay more attention to it. It is possible to provide some setup instructions in \textit{setup\_instruction} that help the model collect the information required to generate the test successfully. In our case, we only use this placeholder when testing the \textit{GCDM Customer} API to provide an example of how to make a login request to the system. This showcases the adaptability of the solution in different use cases. Lastly, we provide the API specification in the \textit{api\_specification} placeholder. The API is expected to have a bigger context of all the input, so it comes in last so that the model does not miss any relevant information.

    \item \textbf{GenAI Model}: This tool connects all the generative AI models. It receives both system and user prompts and sends them to the LLM selected by the user. In our solution, we have used the default \textit{temperature} and \textit{top\_p} values, both at 1. The tool is then expected to return the content generated by the model so that we can continue the flow execution. 
    
    \item \textbf{Parse Generation}: Receives the output of the LLM and parses it to a JSON structure. This script basically searches for the tags specified on the System Prompt Output Structure and joins the content into a single string that will be added to the respective JSON element, see Figure~\ref{fig:systemPromptOutputStrucuture}.
    \end{itemize}

\subsection{Test Execution Module}

Figure~\ref{fig:execution} showcases the internal logic of the Test Execution flow. Tests are expected to be deterministic, so consecutive flow runs with the same test are expected to produce the same result. This flow is executed inside a nodejs environment capable of executing Typescript processes that run tests that use the Jest and Axios libraries. The environment should also contain the environment variables populated for executing the test. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\linewidth]{figures/executionFlow.pdf}
    \caption[Execution Flow.]{Execution Flow. Showcases the processes involved in the automated execution of a test case and the respective result collection.}
    \label{fig:execution}
\end{figure}

Following is a description of each script used in the flow:
\begin{itemize}
    \item \textbf{Save Test to File}: The code generated by the LLM comes formatted in a markdown code block. This script basically parses the code block and writes it to a file inside the execution environment in pure Typescript without any markdown syntax.
    
    \item \textbf{Execute Test}: With the test written to a file, we can now execute the test and collect the report. To do so, we launch a new process that executes a node command \textit{npx jest --json <file>}. The execution may resolve in two ways: \textit{ERROR} or \textit{RUN}. \textit{ERROR} happens when the process cannot execute the file containing the code. For example, the file may not contain any code due to a hallucination on the LLM that did not generate any code. On the other hand, \textit{RUN} happens when the process can execute the code in the file. Of course, the code may still have syntax or semantics errors, but that analysis comes in later phases. Lastly, the script collects other metrics that came from a JSON report in the \textit{parse json report} phase. This includes the total number of tests, the number of tests that passed, the number of tests that failed, and the failing message, if any.
\end{itemize}

\subsection{Test Refactoring Module}

Figure~\ref{fig:refactoring} showcases the internal logic of the Test Refactoring flow. Similar to the Generation flow, consecutive runs of the Refactoring flow with the same data may produce different results due to the creativity of the LLMs. The main purpose of this flow is to iterate over a previously generated test to improve it. It accepts improvement instructions provided by the user or execution errors previously collected. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\linewidth]{figures/refactoringFlow.pdf}
    \caption[Refactoring Flow.]{Refactoring Flow. Showcases the flow of data in the refactoring process of a test.}
    \label{fig:refactoring}
\end{figure}

Following is a description of each script used in the flow:
\begin{itemize}
    \item \textbf{Chat History}: Array of previous interactions with the LLM. This includes the initial system prompt, followed by the initial user prompt and respective generation. These first three elements are then followed by any number of refactoring prompts and respective LLM generation. Figure~\ref{fig:chatHisotryTemplate} showcases a template of chat history with a single refactoring prompt. The chat history is useful since it contextualizes the model on what it has previously generated. 
\begin{figure}[h!]
    \begin{lstlisting}[style=json]
{
    "system_prompt": <system_prompt_placeholder>,
    [
        {
         "user_prompt": <user_prompt_placeholder>,
         "generation": <generation_placeholder>
        },
        {
         "user_prompt": <refactoring_prompt_placeholder>,
         "generation": <generation2_placeholder>
        }
    ]
}
\end{lstlisting}
    \caption[Chat History template.]{Chat History template. Contains the system prompt and an array with all the interactions with the model.}
    \label{fig:chatHisotryTemplate} 
\end{figure}
    
    \item \textbf{Refactor Prompt}: Provides information useful for the LLM to refactor or improve the test and arrive at an improved test generation. Figure~\ref{fig:refactoringPrompt} showcases the latest refactoring prompt in use. At first, we provide the error log in the \textit{error} placeholder so that the model can know why the test has failed. The errors can be very diverse, so we trust the model reasoning capabilities to interpret them and arrive at a possible solution. Following, we provide the model with the user improvement instruction in the \textit{user\_instruction} placeholder. This information can range from providing experimental data to the model to guiding the model to reason about other cases. Once more, the user can provide the information that he finds beneficial.
\begin{figure}[h!]
\begin{lstlisting}[style=prompt]
The test that you have generated has given an error when executed in the Jest environment. 
I want you to refactor the test and generate valid typescript code that can be executed.

First, you will read an error log that describes the error raised upon execution.
This serves as a guideline for you to make appropriate fixes to the previous test. 
Here is the error log:
***
{{error}}
***
{{user_instruction}}
You will now generate the executable typescript test. Let's start!
    \end{lstlisting}
    \caption[Refactoring Prompt Structure.]{Refactoring Prompt Structure. Details of the prompt structure passed to the LLM, with placeholders for the error log and the user-provided instructions.}
    \label{fig:refactoringPrompt} 
\end{figure}
    
    \item \textbf{GenAI Model}: It is the same tool used in the Test Generation flow that connects to all the generative AI models. It receives both the chat history and refactoring prompt and sends them to the LLM selected by the user. Once more, we have used the default temperature and top\_p values, both at 1. The tool is then expected to return the content generated by the model so that we can continue the flow execution.
    
    \item \textbf{Parse Generation}: Despite the refactoring process, the output is expected to be the same, containing the three tags specified in the System Prompt Output Structure, see Figure~\ref{fig:systemPromptOutputStrucuture}. Therefore, this parser receives the output of the LLM and creates a JSON object with all the information.
\end{itemize}


\section{Prompt Engineering}  \label{sec:promptEngineering}
%TODO Evolution of the prompt over time.
%TODO System prompt
%TODO User Prompt

In the realm of generative AI, prompt engineering plays a critical role in achieving the expected results. This section explains various techniques related to prompt engineering that we have used to improve our solution. For that, we start by exploring some guidelines that the user should follow when constructing the business requirement prompt.

Returning to Figure~\ref{fig:APIMatrix}, it describes three levels of prompts, each associated with some quadrant. Prompt L1 is associated with two of them, while prompt L2 and L3 are associated with the two missing quadrants. The meaning of each prompt level is as follows:
\begin{enumerate}
    \item \textbf{LEVEL 1: Basic Requirement Description}
        \begin{itemize}
            \item \textbf{Scope}: This level expects a description of the business requirement using a user story structure. For example, \textit{ As [user description], I Want [functionality], so that [benefit]}.
            \item \textbf{Complexity}: This prompt level works well in APIs with low restrictions and complexity.
            \item \textbf{Documentation}: The documentation may vary from simple to detailed since the LLM has the capacity to make correct assumptions.
        \end{itemize}
    
    \item \textbf{LEVEL 2: Experimental Data Inclusion}
        \begin{itemize}
            \item \textbf{Scope}: Level 2 extends the Level 1 prompt by providing experimental data to be used in the request made to the API. This data can be, for example, a list of valid values to use in a request parameter. Describing a relation between inputs and expected outputs can also help the LLM.
            \item \textbf{Complexity}: This prompt level improves the tool performance in APIs with higher restrictions and complexity.
            \item \textbf{Documentation}: The documentation must be very detailed and complete, allowing the LLM to make correct connections and reasoning.
        \end{itemize}
    \item \textbf{LEVEL 3: Comprehensive Guiding Information}
        \begin{itemize}
            \item \textbf{Scope}: Level 3 requirements build on Level 2 by adding guiding information, such as test plans, acceptance criteria, or tips to use the API resources.
            \item \textbf{Complexity}: This prompt level can perform well in APIs with higher restrictions and complexity.
            \item \textbf{Documentation}: This prompt level can compensate for simpler API documentation since we are providing more context on how to use the resources of the API. 
        \end{itemize}
\end{enumerate}

A significant limitation of current LLM models is their context window size. For data-dependent applications like ours, the small context windows of some models cannot accommodate all the information we need to provide. In our solution, we overcame this challenge by making use of RAG. See Figures~\ref{fig:RAGdatabase} and \ref{fig:RAG} for more details.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/databaseRAG.pdf}
    \caption[RAG database construction.]{RAG database construction. Showcases the process of constructing a vector database from an API specification.}
    \label{fig:RAGdatabase}
\end{figure}

To be able to use RAG, we first need to create a vector database to store our data. The data we are referring to is the API specification, and Figure~\ref{fig:RAGdatabase} shows the steps that we take to process and store it. Given an API specification in JSON format, we input it into a \textit{JSON splitter} to cut it into smaller chunks with a minimum size of 800 tokens and a maximum size of 1200 tokens. According to our own analysis, this range of chunk size is extensive enough to keep related information all together and small enough to keep the chunk data objective. To do this job, we used Langchain Recursive Json Splitter~\hyperfootnote{https://api.python.langchain.com/en/latest/json/langchain_text_splitters.json.RecursiveJsonSplitter.html}{foot:jsonSplitter} that divides the input into chunks in a hierarchical and iterative manner using a set of separators~\cite{ref:recursiveChunking}. After obtaining the different chunks of the API we send them to the ada embedding model to obtain their vector representation. With the embeddings and documents at hand, we construct the database to hold all the data and allow us to search for similar documents. We use the ChromaDB database, which can be executed in memory, making the system easier to deploy.

With an embedding database populated and running, we can start using it to search for similar documents. Figure~\ref{fig:RAG} provides an overview of the whole process.
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/RAG.pdf}
    \caption[RAG.]{RAG. Showcases the full RAG process, from receiving the requirement, creating the vector store index, and searching for similar documents in the database.}
    \label{fig:RAG}
\end{figure}
Given a requirement, we start by expanding it using the \textit{Requirement Expansion} script. This script utilizes an LLM to generate various versions of the requirement, each with a different perspective. With this transformation, the business requirement is kept the same since we request the LLM to rephrase the text using similar but different words.
Once we have all the expanded versions, we can generate their embeddings using the ada embedding model, which was also used to build the database. 
Next, we create a vector store index to find document chunks related to our requirement. Since we have multiple versions of the same business requirement, a set of relevant documents is retrieved for each version. We then perform a unique union across all retrieved chunks to obtain a larger set of potentially relevant chunks. 
By generating multiple perspectives of the same requirement, we can overcome some limitations of distance-based retrieval, resulting in a richer set of results. Finally, we are left with the most relevant parts of the API specification, the \textit{API context}, which we can add to the prompt of the LLM. 
Hallucinations have a low impact on this process since the outcome is a set with a union of all retrieved chunks. The original requirement version is also used when retrieving the documents, so the prompt will always receive relevant documents. 

Thanks to the modularity of our solution, we can combine our flows in multiple ways, allowing us to adapt to different scenarios. We recommend two primary approaches for using our tool: the chain of thought~\cite{ref:chainOfThoughts} approach and the tree of thought~\cite{ref:treeOfThoughts} approach.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/chainOfThought.pdf}
    \caption[Chain of thought approach.]{Chain of thought approach. It consists of executing any number of refactoring test flows after an initial execution of the generate test flow.}
    \label{fig:chainOfThought}
\end{figure}

Figure~\ref{fig:chainOfThought} shows how the chain of thought approach can be used. It basically consists of linking each new test directly to the one before it, forming a chain. To do that, we first generate an initial test with the \textit{Generate Test} flow, then using the \textit{Refactor Test} flow, we iterate over the test to generate multiple versions of it. In our case, the business requirement is the idea that connects every test. The chain approach provides coherent and contextually relevant tests when used in a short context. However, when the chains start to increase, it may get lost, effectively reducing the relevance of the generated tests.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\linewidth]{figures/treeOfThought.pdf}
    \caption[Tree of thought approach.]{Tree of thought approach. It consists of executing the generate test flow several times to get various test cases.}
    \label{fig:treeOfThought}
\end{figure}

Figure~\ref{fig:treeOfThought} shows how the tree of thought approach can be used. This approach organizes the tests into a tree-like structure, with each business requirement branching off into multiple related tests. To do that, we basically execute the \textit{Generate Test} flow multiple times with similar inputs. The user may make small changes to the business requirement input to steer the generated tests in the desired direction. In longer contexts, the tree approach is often better at maintaining the coherence of ideas.

\section{Solution prototype} \label{sec:solutionWorkflow}

We have created a user interface (UI) using the Streamlit framework to ease the user's interactions with the flows. This serves as a prototype to showcase the feasibility of the solution and provides an example of how it could be integrated into a production environment. This interface also facilitated our interactions with the flows during the validation process. The solution can be divided into three main components: Input, Data, and Results. See Figures%~\ref{fig:loadUI},
~\ref{fig:inputUI},~\ref{fig:dataUI}~and~\ref{fig:resultsUI}, respectively, to know their structure.

%\begin{figure}[h!]
%    \centering
%    \frame{\includegraphics[width=1\linewidth]{figures/loadUI.pdf}}
%    \caption[Load UI.]{Load UI. Interface to load files storing data from previous runs.}
%    \label{fig:loadUI}
%\end{figure}

%Figure~\ref{fig:loadUI} shows the interface to load a run into the solution. The key components are the following: 
%\begin{itemize}
%    \item \textbf{Clone Button}: Clones the current run into a new file.
%    \item \textbf{Run Drop-down}: Lists all the available files with run data.
%    \item \textbf{Load Button}: Loads the data from the selected file.
%\end{itemize}

\begin{figure}[h!]
    \centering
    \frame{\includegraphics[width=1\linewidth]{figures/inputUI.pdf}}
    \caption[Input UI.]{Input UI. Interface to receive user inputs and select tools and processes to use in the generate test flow.}
    \label{fig:inputUI}
\end{figure}

Figure~\ref{fig:inputUI} shows the interface to collect the inputs for the run. The key components are the following: 
\begin{itemize}
    \item \textbf{Business Requirement Text Box}: Collects the description of the business requirement to test. It can also receive a oneShop user story ID in the format \textit{SHOP-0000}.
    \item \textbf{Service Drop-down}: The name of the API being tested. When expanded, it lists all the API specifications we can test. 
    \item \textbf{API process type Drop-down}: Methods used to process the API specification. When expanded, it shows all available API processing methods, either RAG or Full. Refer to Figure~\ref{fig:generation}.
    \item \textbf{LLM Model Drop-down}: LLM used to generate the test. When expanded, it shows all the available LLMs.
\end{itemize}

\begin{figure}[h!]
    \centering
    \frame{\includegraphics[width=1\linewidth]{figures/dataUI.pdf}}
    \caption[Data UI.]{Data UI. The interface displays the API specification in use, prompts sent to the LLM, and generation received from the LLM, with metrics of the number of tokens and time to generate.}
    \label{fig:dataUI}
\end{figure}

Figure~\ref{fig:dataUI} displays the data used in the run and respective metrics. The key components are the following: 
\begin{itemize}
    \item \textbf{API Expander}: When expanded, displays the API specification in use.
    \item \textbf{System prompt Expander}: When expanded, displays the system prompt sent to the LLM.
    \item \textbf{Prompt Expander}: When expanded, displays the user prompt sent to the LLM. More prompt expanders appear after a call to the refactor flow.
    \item \textbf{Generation Expander}: When expanded, displays the output generated by the LLM. More generation expanders appear after a call to the refactor flow.
    \item \textbf{Tokens Field}: Total number of tokens associated with the data.
    \item \textbf{Time to generate Field}: Number of seconds taken to process all the data and generate a response.
\end{itemize}

\begin{figure}[h!]
    \centering
    \frame{\includegraphics[width=1\linewidth]{figures/resultsUI.pdf}}
    \caption[Results UI.]{Results UI. The interface displays the generated test and the results obtained upon test execution. It gives access to buttons that can launch the execute and refactor flows and an input box to receive additional user instructions.}
    \label{fig:resultsUI}
\end{figure}

Figure~\ref{fig:dataUI} provides access to the generated test and the corresponding results. The key components are the following: 
\begin{itemize}
    \item \textbf{Test Expander}: When expanded, the generated test is displayed in a well-formatted and organized manner. An option to edit the test is also made available for the user.
    \item \textbf{Execute Button}: Triggers the execution of the Execute Test flow that will run the test in the nodejs environment.
    \item \textbf{Test Error Radio Button}: User-provided input that describes the type of error that occurred.
    \item \textbf{US Level Radio Button}: User-provided input that describes the prompt level, according to the description on Section~\ref{sec:promptEngineering}.
    \item \textbf{Save Button}: Saves the user provided information.
    \item \textbf{Number of tests Field}: Total number of tests in the test script.
    \item \textbf{Pass tests Field}: Number of tests that pass after execution.
    \item \textbf{Fail tests Field}: Number of tests that fail after execution.
    \item \textbf{Run Expander}: Output generated from executing the test. All the error messages will be shown when the component is expanded.
    \item \textbf{Optional Instruction Text Box}: Collects the instructions that the user may want to provide when executing the refactoring flow.
    \item \textbf{Refactor Button}: Triggers the execution of the Refactor Flow that generates a new test based on the current one.
\end{itemize}

\section{Summary}

In this chapter, we presented APITestGenie, an innovative tool designed to help users autonomously create API integration tests efficiently. The chapter details the tool's data usage, key technologies, architecture, prompt engineering techniques, and a solution prototype.

Using the right data is crucial for APITestGenie. Data collection involved creating pipelines to automate the processes of collecting, cleaning, and filtering relevant data. The data collected included business requirements from user stories, sequence diagrams, and OpenAPI specifications. Various sources, such as project management tools and technical documentation, were used to retrieve business requirements. Additionally, various OpenAPI specifications were collected and processed to validate the solution across different environments and constraints.

The key project technology is LLMs, which initially started with LLAMA2 but later shifted to GPT for better performance. Azure services used include OpenAI Studio and Machine Learning Studio. Python libraries like LangChain, ChromaDB, Tiktoken, and Streamlit were essential. Cost and performance considerations led to the choice of GPT-4-Turbo. A nodejs environment with Jest and Axios libraries was set up to validate the generated tests.

The architecture is divided into three main flows: Test Generation, Test Refactoring, and Test Execution. Each flow involves different processes, inputs, outputs, and tools. The Test Generation flow creates the test, Test Execution provides results, and Test Refactoring iterates over the test to improve it. The modular approach allows flexibility in execution.

Prompt engineering is critical for achieving the expected results. Three prompt levels were defined based on API complexity and documentation detail. Techniques like RAG were used to handle large API specifications. The solution can combine different flows to adapt to various scenarios using chain-of-thought or tree-of-thought approaches.

A prototype using Streamlit was created to demonstrate a possible solution UI. The interface includes components for loading files, collecting user inputs, displaying data and results, and executing flows. This prototype showcases the feasibility of the solution and provides an example of how it could be integrated into a production environment.

==> Tese_Andre/chapter4.tex <==
\chapter{Validation} \label{chap:results}

This chapter aims to validate our tool and comprehensively analyze the results. To do so, we performed two distinct validations. The first validation activity, presented in Section~\ref{sec:performanceExperiment}, analyzes the tool performance, and we collected metrics to validate the syntax and semantic correctness of the tests.
In the second validation activity, presented in Section~\ref{sec:useCaseExperiment}, we conducted a practical workshop to demonstrate the capabilities of APITestGenie using real data from Critical Techworks. Our target audience comprised technical experts with extensive experience in the product. This approach enabled us to gather valuable feedback on the test's relevance and completeness. Section~\ref{sec:discussion} lists our key findings and provides an answer to our research question. In Section~\ref{sec:limitations}, we discuss the current limitations of the tool.
In both experiments, we used GPT-4-Turbo, version 1106-Preview, with a context window of 128k.

\section{Performance Experiment} \label{sec:performanceExperiment}
%Manually performed tests
%Syntax correctess (100% ok)
%Semantics correctness (value in assert is ok)

With this first experiment, we aim to validate the robustness of the APITestGenie. We used various data sources to ensure the tool could be used in diverse environments. 

\subsection{Experimental Setup}

For the first experiment, we used 25 distinct inputs. The inputs were collected from the documents made available by the company. An input is composed of an API specification and a business requirement. We executed the generative process three times for each input so that we could later calculate the pass@k metric. This resulted in 75 generated tests. Table~\ref{tab:generationByService} shows the distribution of generations by service. Bigger and more complex APIs, see Figures~\ref{fig:apiSpecification}~\ref{fig:APIMatrix}, provide more insights on top of having more business requirements, so more tests were generated for them. The used APIs are a great example of services found in real-world applications. 
\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
        Service & Number of Tests \\ \hline
        Cat Fact & 3 \\
        Pet Shop & 6 \\
        GCDM Customer & 6 \\
        GCDM & 6 \\
        OneShop & 6 \\
        UCP Accessories & 6 \\
        UCP Otd & 15 \\
        UCP Localisations & 6 \\
        UCP Vehicles & 12 \\
        UCP All & 9 \\
    \end{tabular}
    \caption{Number of generations by Service}
    \label{tab:generationByService}
\end{table}

Table~\ref{tab:generationByPromptLevel} shows the distribution of generations by prompt level. We aim to use various prompt levels in the generations to validate their implications in experiments with distinct characteristics. L1 prompts were easier to collect, which justifies their higher representativity. Nevertheless, we tried to balance the dataset with L2 and L3 prompts. However, the number of tests for each prompt level is constrained by the business requirements in the company's documentation.

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
        Prompt Level & Number of Tests \\ \hline
        Level 1 & 33 \\
        Level 2 & 18 \\
        Level 3 & 24 \\
    \end{tabular}
    \caption{Number of generations by Prompt level}
    \label{tab:generationByPromptLevel}
\end{table}

Figure~\ref{fig:generationLevelService} shows the distribution of the generations of each prompt level by service. More complex services tend to have more complex prompt levels. On the other hand, simpler services tend to have simpler prompt levels. Appendix~\ref{apx:publicRuns} shows the business requirement and respective generation obtained in the nine runs of the \textit{Pet Shop} and \textit{Cat Fact} services. The remaining runs follow the same behavior. However, we can not show the associated data due to data privacy constraints.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures/generationLevelService.pdf}
    \caption{Number of runs for each prompt level by service}
    \label{fig:generationLevelService}
\end{figure}

In each run, we collected metrics, such as the time taken to generate the test, the number of tokens used, the number of tests, the number of passed tests, and the number of failed tests. When the test did not pass, we manually categorized the error into five types:
\begin{itemize}
    \item \textbf{Syntax}: The typescript code generated is syntactically incorrect.
    \item \textbf{Semantics}: The data used in the test does not make sense. For instance, data used in assertions is incorrect.
    \item \textbf{No Test}: Generation has no test or code.
    \item \textbf{Permission}: Test execution failed due to insufficient permissions to API resource.
    \item \textbf{Defect}: Tests that do not pass. However, according to the API specification, they are valid.
\end{itemize}

\subsection{Experimental Results}

In the data used, the mean input tokens of the tests were 35,289, and the mean output tokens were 698. According to the prices listed in Table~\ref{tab:gptPricing}, generating all 75 tests cost 28€, with a mean price of 0.37€ for each generation.

Figure~\ref{fig:codeGenerated} shows that most runs could generate Typescript code. This demonstrates the capability of the tool to address our problem needs. In the run that resulted in no code, the LLM generated an output explicitly stating its incapacity to understand the business requirements, see Appendix~\ref{apx:noCode}. This is a type of error that can occur when using the tool. Nevertheless, we still believe that the LLM output was relevant to the user as it provided insights into what went wrong. In the other two similar runs, the LLM successfully generated code.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/codeGenerated.pdf}
    \caption[LLM generated code.]{LLM generated code. In 75 runs, 74 generated code, while 1 did not.}
    \label{fig:codeGenerated}
\end{figure}

For the tool to be useful, it must generate a response in an acceptable time. Figure~\ref{fig:timeToGenerate} relates the number of input tokens to the time taken to generate a response. As the regression line indicates, the increase in the number of input tokens increases the time needed to generate a test. The time can range between 43 seconds for a prompt with 5,071 tokens and 266 seconds for a prompt with 70,539 tokens. The increase is not proportional between the two parameters since the generation time increases almost six times, while the number of tokens in the input prompt increases by more than 14. Additionally, for the same number of tokens, the generation time also varies. This relates to the Azure services used since our inputs are the same. Given the amount of information we are dealing with, we believe the time range is acceptable since the tool can work autonomously in the background without demanding attention from the user. We have not considered the output tokens in this analysis since their sizes are similar when the inputs are the same. Additionally, the number of output tokens is much less than the input tokens, which does not influence the representation.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures/timeToGenerate.pdf}
    \caption[Number of tokens VS Time to generate.]{Number of tokens VS Time to generate.}
    \label{fig:timeToGenerate}
\end{figure}

To validate the content of the generated test script we felt the need to analyze the tests upon their execution. Figure~\ref{fig:testCaseResult} shows the results. The 75 test generation runs ended up generating 90 unique test cases, from which more than half passed, 55.1\%, and the rest, 44.9\%, failed. Since we are testing the business requirements of systems in production, most of the tests are expected to pass. These results are somewhat doubtful, so we decided to explore the reasons that resulted in the failure of 40 test cases.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/testCaseResult.pdf}
    \caption[Test case execution result.]{Test case execution result. Number of passed and failed test cases after script execution.}
    \label{fig:testCaseResult}
\end{figure}

Figure~\ref{fig:errorTypes} categorizes the failed tests using the previously defined error types.
The \textit{syntax} errors are mainly due to placeholders that the model leaves in the generated code for the user to complete or variables with incorrect scope. The test structure is correct when syntax errors occur, but the user must make a few changes to execute the test. Generations with \textit{syntax} error type and \textit{no test} error type contain zero test cases. This means that 4 of the generations have 0 test cases. 
The \textit{permission} error type occurs in 7 generations when a resource can not be accessed, resulting in a \textit{403 Forbidden} error upon the test execution. 
The \textit{defect} error type occurs in 11 generations when a test assert throws an error or when a requested resource was not found, resulting in a \textit{404 Not Found} error. However, according to the API specification, the data used is correct in both cases. We could not validate the issue further since we could not access the source code.
Lastly, the \textit{semantic} error type occurs in 22 generations, so we felt the need to expand it further into three subcategories as follows: 
\begin{itemize}
    \item \textbf{Hallucination}: Test script contains incorrect assumptions and uses wrong data.
    \item \textbf{API outdated}: Generation uses deprecated resources.
    \item \textbf{Other}: Miscellaneous, missing information, unable to structure request.
\end{itemize}

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/errorTypes.pdf}
    \caption[Frequency of errors types.]{Frequency of errors types in failed executions.}
    \label{fig:errorTypes}
\end{figure}

Figure~\ref{fig:semanticErrorTypes} shows the distribution of semantic error types. Most of the errors, 19, are due to \textit{Hallucinations} of the LLM. The reason for the errors are the following:
\begin{itemize}
    \item Wrong or nonexisting imports.
    \item Data types manipulation errors, for instance, date objects.
    \item Wrongly built resource URLs.
    \item Assumption of resource attributes that do not exist.
    \item Access to object unexisting attributes.  
    \item Wrong interpretation of the response structure.
\end{itemize}
Additionally, we had one occurrence of a \textit{API outdated}, where the model used a deprecated resource. We consider it a semantic error type since requesting this endpoint does not make sense since it was discontinued.
Lastly, we had two semantic error tests categorized as \textit{others}, where the reason for the error is due to missing information in the API specification, which makes it impossible to structure the request. We can conclude that semantic error types result from the lack of capabilities of the LLM in use.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/semanticErrorTypes.pdf}
    \caption[Frequency of semantic error types.]{Frequency of semantic error types in semantic errors.}
    \label{fig:semanticErrorTypes}
\end{figure}

Given the above analysis, we consider valid the tests that pass upon execution and those that resolve in error type categorized as \textit{defect} since they are correct according to the API specification. A user that uses our tool is expected to address the defect errors by first validating the API specification and then validating the code implementation that resulted in the error.
% They may have found an error in the API implementation
Figure~\ref{fig:testOutcome} shows the distribution of the test's validity by each API specification. We concluded that less complex APIs tend to have more valid tests, for instance, \textit{Cat Fact}, \textit{GCMD Customer}, \textit{Pet Shop} and \textit{UCP Otd}. This is also related to the prompt level required to generate a valid test. In this case, L1 prompts are enough. For the services that have higher complexity, for instance, \textit{UCP Vehicles}, \textit{UCP Localisations} and, \textit{GCDM}, the L1 prompt level is sometimes not enough to generate a valid test. Therefore, writing more complete prompts is a requirement to generate a higher number of valid tests. Lastly, \textit{Oneshop} and \textit{UCP All} are the services with the highest number of invalid tests. In both cases, we only used L3 prompts. This highlights the LLM's difficulty interpreting their specifications. The \textit{OneShop} complexity is due to its limited and simpler documentation. The \textit{UCP ALL}, despite having a complete and well-documented API its size requires the use of RAG, which summarizes a lot of information, adding more uncertainty to the process.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/testOutcome.pdf}
    \caption[Test validity by service.]{Test validity by service.}
    \label{fig:testOutcome}
\end{figure}

Using the pass@k metric from the HumanEval\cite{ref:humanEval}, we tested the validity of our tests for $k = \{1,2,3\}$. The initial 75 runs resulted in 25 runs. Figure~\ref{fig:passk} shows the results obtained. Overall, the probability of generating a valid test increases in successive generations. Comparing prompts \textit{L1} and prompts \textit{L2}, which are both used in the same API services, we can conclude that \textit{L2} prompts achieve better results. This behavior is expected since we are providing experimental data to the LLM, reducing the occurrence of semantic errors. Prompts \textit{L3}, which are mainly used with more complex API services, such as \textit{OneShop} and \textit{UCP All}, do not show as much improvement in successive generations. The complexity of API and business requirements is the reason why L3 prompts perform worse than other prompt levels. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/passk.pdf}
    \caption[Pass@k test validity.]{Pass@k test validity. \textit{All} is the mean of all three prompt levels.}
    \label{fig:passk}
\end{figure}

To further explore the implications of the API characteristics when generating tests, Figure~\ref{fig:pass3ByService} shows pass@3 test validity by service. We concluded that for most inputs, when executing the generation process three times, the LLM was able to generate at least one valid test. The reasons for the results of \textit{OneShop} and \textit{UCP All} APIs are related to their complexity and level of documentation details, as explored before. However, \textit{UCP Accessories} appears in the figure with an invalid test. The reason is that we only use prompts L1 in an API where the use of prompts L2 is recommended. With this analysis, we can conclude that the tool is capable of generating valid tests given the proper inputs.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/pass3ByService.pdf}
    \caption[Pass@3 by service.]{Pass@3 by service.}
    \label{fig:pass3ByService}
\end{figure}

Lastly, we felt the need to validate the benefits of using RAG to process the API specification. Therefore, in addition to the 75 already executed runs, we executed 12 more runs against the \textit{UCP Vehicles} with the same inputs. This API is the only one that makes sense to test since it has the specification big enough for the RAG to produce some benefits and small enough to fit in the LLM context window, allowing its use with both strategies. Figure~\ref{fig:benefitsRAG} shows our findings. Despite not being very notorious, the RAG strategy produces more valid tests while reducing the number of input tokens. In this experiment, the conditions for a valid test are the same as before. The tests considered in the 75 generations set are the ones that use the RAG strategy.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/processingAPI.pdf}
    \caption[Test validity using RAG.]{Test validity using RAG. Runs executed against UCP Vehicles API with the same inputs only change the API processing strategy.}
    \label{fig:benefitsRAG}
\end{figure}

\subsection{Experimental Conclusions}

To conclude, the high complexity of the API influences the results obtained when generating test cases. However, the tool's performance can be increased if we have good documentation and business requirement descriptions adapted to the APIs under test. From the 75 generated tests, 56\% were valid. In the failing tests, we identified that the problems were not related to syntax errors, which was correct in most test scripts. The majority of the problems are related to semantic problems. Since semantic errors are related to the data used, the test structure is still useful for the user, with an initial starting point and ideas to test. Furthermore, we can use the presented strategy of generating a test three times for the same input to arrive at a test validity of 80\%. Lastly, using RAG provides a way to optimize the contextual information sent to the LLM, allowing us to overcome its strict context size. This experiment was very successful as it proved the robustness of APITestGenie.

\section{Company Use Experiment}\label{sec:useCaseExperiment}

In the second experiment, we moved to a more practical validation that relied on a presentation of APITestGenie to technical staff from Critical Techworks, followed by a feedback form. The present staff members have daily contact with product development, which makes them capable of evaluating the generated tests regarding their relevance and completeness. On top of that, they are highly contextualized with the services and resources used in the presentation examples.

\subsection{Experimental Setup}

The presentation started with a brief context and solution description followed by two practical examples. The first example showcases a progressive run against \textit{UCP Otd} API, where the user adds more information to the business requirement in successive runs. Here, we aim to show how changes to the business requirement affect the generated test. Figures~\ref{fig:progressiveRun1}, \ref{fig:progressiveRun2}, \ref{fig:progressiveRun3} show all three business requirements used in this first example. Appendix~\ref{apx:progressiveRun} shows the generations obtained in each run.

\begin{figure}[h!]
    \begin{lstlisting}[style=prompt]
As a user I want to retrieve all the countries where the service is available.
    \end{lstlisting}
    \caption[Progressive run 1º example.]{Progressive run 1º example. Prompt Level 1 basic description}
    \label{fig:progressiveRun1} 
    \begin{lstlisting}[style=prompt]
As a user I want to retrieve all the available ag-models in the eu27+ country so that I can know which vehicles are available.
    \end{lstlisting}
    \caption[Progressive run 2º example.]{Progressive run 2º example. Prompt Level 2 provides experimental data.}
    \label{fig:progressiveRun2} 
    \begin{lstlisting}[style=prompt]
As a user I want to retrieve all the existing country codes then select one so that I can retrieve all the available ag-models for the country so that I can know which vehicles are available.
    \end{lstlisting}
    \caption[Progressive run 3º example.]{Progressive run 3º example. Prompt Level 3 provides guiding tips.}
    \label{fig:progressiveRun3} 
\end{figure}

The second example showcases a business requirement that uses multiple resources of \textit{UCP All} API. In this example, we aim to provide an overview of the complexity the tool can handle. Figure~\ref{fig:complexRun} presents the business requirement used, and Appendix~\ref{apx:complexRun} shows the respective generation.

\begin{figure}[h!]
    \begin{lstlisting}[style=prompt]
As a user I want to retrieve the price of acessories for a bmwCar in the italian market. 

First test, using /vehicles service get a list of all available vehicles models in the market and select a random model. 
Second test, using /accessories service and with the model previously selected retrieve the list of all available accessories on the 17/05/2024.
Third test, using /pricing service to retrieve the calculated price of the available car accessories in the pcaso,con priceListsIdentifiers.
    \end{lstlisting}
    \caption[Complex run.]{Complex run. Prompt Level 3 provides guiding tips on how to structure the test.}
    \label{fig:complexRun} 
\end{figure}

The feedback form was answered right after the presentation and was divided into two sections. The first section contained demographic questions, which are the following:
\begin{enumerate}
    \item What's your role in CTW?
    \item How many years of experience do you have in your current role?
    \item How often do you have the need to create integration tests?
\end{enumerate}

The second section contained affirmations and questions which we asked the staff to answer based on their opinion on the solution results, which are the following:
\begin{enumerate}
    \item The purpose of the tool is clear to me.
    \item The information required by the tool (swagger + requirement) is easily accessible.
    \item I am satisfied with the relevance of the tests generated by the tool.
    \item I believe the tool was able to cover various aspects of the business requirement.
    \item I believe the generated tests can be immediately integrated in a testing environment.
    \item I believe the tool can accelerate the process of creating tests compared to manual testing.
    \item Security-wise, I believe the tool can be safely used in an enterprise context.
    \item How likely are you to use the tool in your day-to-day work?
    \item Additional comments that you would like to share?
\end{enumerate}

\subsection{Experimental Results}

This section shows the results obtained in the use case experiment. Figures~\ref{fig:roleCTW} and \ref{fig:experienceCTW} provide an overview of the staff competencies to which we have presented our solution. We counted the participation of 15 collaborators in the presentation section and collected 11 answers in our forms. The missing 4 persons did not feel comfortable responding to the feedback form.

Figure~\ref{fig:roleCTW} shows the roles the inquiries take in Critical Techworks. Most of them are Rockstar developers, meaning they are responsible for developing code and product features. We also have Scrum Knights that accumulate both the Rockstar developer responsibilities and the management of the team's agile processes. One Product Visionary, who is not directly related to the code development, is responsible for collecting the business requirements of the product. All of them have some impact on tool components.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/roleCTW.pdf}
    \caption{Roles in Critical Techworks.}
    \label{fig:roleCTW}
\end{figure}

Figure~\ref{fig:experienceCTW} shows the experience in years of the inquiries in the current role. The mean is around five years, which we believe is enough experience to meet our needs. During all these years, the inquiries have been working on the project we are testing, which provides them with a lot of business knowledge.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/experience.pdf}
    \caption{Years of experience.}
    \label{fig:experienceCTW}
\end{figure}

In Figure~\ref{fig:frequencyCTW}, we explore the frequency the collaborators need to create integration tests. Most of the answers float around \textit{Weekly} and \textit{Monthly}. This is expected since integration tests tend to be more complex to develop and aim to test a service's business requirement, which normally takes more than one day to develop. What's more, is that one of the staff members who responded \textit{Never} is the Product Visionary who is not involved in development activities. After further conversation to understand the other responses, we discovered that creating unit tests is more common than creating integration tests. However, there is a general interest in the company in increasing the number of integration tests available. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/frequencyTests.pdf}
    \caption{Frequency to create integration tests.}
    \label{fig:frequencyCTW}
\end{figure}

Upon this preliminary analysis of the inquiries demographics, Figure~\ref{fig:believesCTW} shows the staff opinion on some affirmations related to the tool. First of all, most of the staff understood the tool's purpose, which is required to answer the following affirmations. 
According to the responses obtained to the second affirmation, we can conclude that the tool is relatively easy to use since the inputs are easily accessible. 
The third affirmation highlights that the tests generated by the tool are relevant, making them useful for the developer. 
Regarding the fourth affirmation, the inquiries arrived at a consensus where all agree that the generated tests are indeed complete and cover various aspects of the business requirement that need to be tested.
The fifth affirmation presents the first unpleasant opinion that states that the test can not be immediately integrated into the testing environment. This is due to the trust factor that the staff currently have in generative AI tools and, as we concluded in the automated experiment, the need for a developer to validate the test content.
However, in the sixth affirmation, there was a strong opinion that this tool could accelerate the process of creating tests, for instance, by creating initial structures detailing what needs to be tested.
Lastly, in the seventh affirmation, while older staff considered the tool less secure, the younger staff considered it acceptable to use. This highlights the interest in setting up secure pipelines and contracts that safeguard the company's interests.

\begin{figure}[h!]
    \centering
    \includegraphics[width=1\linewidth]{figures/believes.pdf}
    \caption{Staff believes of generated tests.}
    \label{fig:believesCTW}
\end{figure}

The final question, which has its results presented in Figure~\ref{fig:likelihoodCTW}, points out the interest from the developers in using the tool in their day-to-day work. More than 50\% of the inquiries are \textit{likely} or \textit{very likely} to use the tool if made available, while the other half is neutral regarding its daily use.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.8\linewidth]{figures/useLikelihood.pdf}
    \caption{Likelihood of using the tool in future.}
    \label{fig:likelihoodCTW}
\end{figure}

The forms ended with an open question, where we collected all the suggestions and comments that Critical Techworks collaborators had, which are the following:
\begin{enumerate}
    \item Can the tool be easily adapted to other technologies?
    \begin{itemize}
        \item[] Yes, the tool can be easily adapted to other technologies by changing the system prompt and providing data related to the new use case.
    \end{itemize}
    \item Usage of the tool to test various test scenarios. For instance, the developer provides an Enum or any other categorical data structure, and the tool could generate tests covering all the categories, considering what is written in the API specification.
    \begin{itemize}
        \item[] This suggestion can be expanded into three different cases. The user may specify the request inputs, and the LLM will try to guess the outputs. The user may specify the output, and the LLM will specify the input. The user may specify both the input and the output, and the LLM will use them in the test. All three cases are valid, which shows the versatility of the tool. On top of that, by giving various inputs or outputs at the same time, the LLM will generate various test cases to cover them all. 
    \end{itemize}
    \item Does the tool require the data specification, or is it creative enough to generate the data autonomously?
    \begin{itemize}
        \item[] Yes, the tool is capable of generating the data autonomously. This autonomous generation is highly dependent on the contents provided on both the business requirements and the API specification. The more information that is provided, the better the tool will behave.
    \end{itemize}
\end{enumerate}

\subsection{Experimental Conclusions}

To conclude, APITestGenie was well accepted by the company collaborators, who showed interest in using the tool. Most collaborators found the tests generated by the tool complete since they covered various aspects of the business requirement and relevant since they tested nontrivial cases. This validates our idea that the tests are indeed useful for the user. Nevertheless, a small group believes improvements are needed to guarantee company data security and immediate integration in a testing environment.

\section{Discussion} \label{sec:discussion}

%Implications of the findings
Given the above analysis, we can conclude that having good documentation and well-defined processes is crucial when using this type of tool to automate manual testing processes. Generative AI relies heavily on data, and ensuring data readiness and availability is the most challenging step. When we began this project, our initial challenge was accessing data. Once resolved, the project progressed smoothly.

From the examples provided, we can conclude that generating tests for highly complex APIs is achievable. The LLM can generate tests for both corner and base cases, depending on the user's request. The key needs are comprehensive documentation and adapted business requirements that provide enough information to guide the LLM in its generation. These requirements may seem challenging, but they are good practices that all developers should follow in their day-to-day work. Although it is not mandatory to match the prompt level to the API complexity, we recommend it to enhance the likelihood of generating valid tests. Additionally, the tool is agnostic to user characteristics since it accepts inputs in various formats. The only constraint is that the input must be logically structured.

Compared to other tools, such as GitHub Copilot~\cite{ref:copilot}, our tool serves a different purpose. While Copilot assists users in real-time as they write code, requiring their interaction, our tool is designed to generate tests for APIs autonomously. This only requires the user to validate the generated test since the creation process can be skipped. Some use cases are the generation of integration tests for existing APIs lacking adequate test coverage or for newly developed API services, enabling faster validation of business requirements. Our tool operates autonomously, requiring only the specification of the business requirement and the API specification to perform its task independently of human intervention.

According to Databricks state of Data + AI~\cite{ref:stateOfAIDatabricks}, 70\% of companies using generative AI use tools and vector databases to augment data models. In our solution, we have used RAG, which heavily relies on a vector database to customize the LLM with the company's private data. Despite not being the same as fine-tuning, RAG is a cheaper and easier way to provide the LLM with relevant information for the task at hand. By using RAG, we achieve less hallucinations and more transparency since we know which documents were used to generate the content.

Given the above analysis, we can now provide an answer to the initial research questions:

\textbf{RQ1: Can we effectively generate integration test cases for an API with LLM?}
\begin{itemize}
    \item[] Yes, our APITestGenie is a practical solution that generates integration tests for an API using an LLM. By inputting business requirements related to various resources, the LLM can produce a comprehensive test script comprising multiple test cases. Each test case targets a specific property, and together, they test the entire flow of the business requirement. Furthermore, given the correct prompt, the LLM can generate test cases to cover different scenario outcomes, both successful and unsuccessful. The clarity of the business requirement prompt is crucial, enabling the LLM to precisely address the user's needs.
\end{itemize}

\textbf{RQ2: Can we effectively generate fuzz test cases for an API with LLM?}
\begin{itemize}
    \item[] Yes, APITestGenie effectively demonstrates the capability to generate fuzz test cases for an API using an LLM. The process involves the user providing a detailed business requirement that outlines the need to test unique and unexpected scenarios. Given the context, the LLM can generate diverse test cases that include a variety of malformed inputs, unusual sequences of API calls, and edge cases that a human tester might not consider. However, take into consideration that without a clear explanation of the fuzz testing need, APITestGenie will solely focus on ensuring the integrity of the business requirement, resulting in the generation of integration tests that validate the correct behavior rather than specific fuzz test cases.
\end{itemize}

\textbf{RQ3: How can prompt-tuned models compare to achieved baseline results?}
\begin{itemize}
    \item[] Several aspects highlight the advantages of prompt-tuned models compared to traditional baseline results. To approach this question, we compare our results with three other perspectives: manually created tests, tool generated tests without generative AI, and LLM generated tests without prompt tuning.

    Firstly, comparing LLM generated tests to manually created tests, one key advantage is enhanced creativity. Due to LLM intrinsic characteristics, this model can generate tests for use cases that manually created tests could not validate. This can be seen as a pair-programming usage helping the user test cases that he has not considered. Furthermore, these models offer greater autonomy, requiring minimal human intervention once appropriately tuned. This autonomy streamlines processes and enables the models to handle more complex tasks independently. Consequently, prompt-tuned LLMs significantly reduce users' workload by generating unique outputs that would otherwise require substantial manual effort.

    Secondly, compared to tool-generated tests without generative AI, prompt-tuned LLMs operate with fewer data restrictions. This flexibility allows for more adaptive and responsive interactions that better match varied user inputs. Moreover, prompt-tuned LLMs are capable of generating more complete tests that include data integrity validations. For instance, QuickRest~\cite{ref:quickRest} generates a test with randomly generated data, without any context while APITestGenie uses data related to the business context. SBST~\cite{ref:gpt_sbst} requires the definition of predefined search approaches, while APITestGenie creates its own testing strategy. RESTTESTGEN~\cite{ref:apiBlackBoxTesting} requires the definition of operation dependency graphs to guess whether a new operation can be tested with the Oracle. APITestGenie is capable of generating various and unique assertions to address each generated test need.
    Tests generation from Bugs ~\cite{ref:testCasesFromBugReport} uses both bug reports and source code, while APITestGenie does not require access to code to generate test cases. Lastly, EvoMaster~\cite{ref:apiAutomatedTestGeneration} generates tests with a focus on code coverage, while APITestGenie aims to validate and guarantee a business requirement in each generated test. We can, therefore, conclude that APITestGenie can adapt to diverse situations autonomously.

    Lastly, when comparing prompt-tuned LLM to LLM-generated tests without prompt tuning, several distinct benefits emerge. One of the most significant advantages is the reduction in hallucinations. Prompt tuning helps direct the model to stay on-topic and provide accurate information, thereby improving the reliability of the outputs. With this research, we concluded that different prompt tuning techniques provide distinct benefits. RAG can increase the amount of information provided to the LLM, while tree-of-thought allows the generation of different versions for the same test. This flexibility is particularly beneficial in adjusting the model’s behavior to specific requirements and contexts. Additionally, prompt-tuned models facilitate automation. By setting up precise prompts, these models can autonomously perform repetitive or complex tasks, enhancing productivity and ensuring a consistent output structure.
\end{itemize}

\textbf{RQ4: Can the industry use the proposed solution to improve resource efficiency?}
\begin{itemize}
    \item[] Yes, it is clear that the industry can and should use this type of tool to improve resource efficiency. These tools are a source of creativity that allows users to achieve results faster and provide ways to automate processes that were previously impossible. The experimental results clearly show that these tools can accelerate the development and delivery of product features. However, security and data privacy remain significant factors that delay the adoption of these technologies. Since the most capable LLMs are provided by major technology companies like Google and OpenAI, there are concerns about how these companies deal with data privacy. Consequently, trust becomes a critical issue and a significant barrier to adopting generative AI tools.
\end{itemize}

\section{Limitations} \label{sec:limitations}

We have identified three primary limiting factors for APITestGenie: the size of the LLM context window, the need for specialized personnel validation, and the costs associated with tool usage.

The context window size of LLMs is a limiting factor of the amount of information we can send to the model. We overcame this constraint with RAG, which filters the relevant data from large API specifications, yielding good results. Additionally, with the launch of Gemini 1.5~\cite{ref:gemini1.5} that has a context window of 2 million tokens, we can see a trend in the LLM landscape to increase the model's context windows, suggesting that this issue will become less significant in the future.

Despite LLMs' creativity and ability to understand tasks, they cannot be fully trusted due to occasional hallucinations that can lead to errors in minor details. Therefore, a specialized person, such as a developer, is still needed to validate the model's outputs. Our experience shows that the structure of the generated test is usually correct, providing a solid starting point and accelerating the creation process. Additionally, a developer can fix existing generated test errors within 2 to 3 iterations, thus speeding up the test development and deployment process. We can conclude, therefore, that technical staff will not be replaced for now since they still have a very important role in maintaining the integrity of the software product.

Lastly, our solution involves processing large amounts of data, particularly API specifications. Depending on the data size, the cost per prompt can be high. For instance, if the company decides to give full access to our tool and each prompt costs approximately €0.37, this can lead to significant expenses over the year. RAG can help reduce the number of input tokens, but it is not a perfect solution as it might omit relevant information. Despite all this, LLMs are becoming more efficient and optimized over time, leading to reduced costs. For example, the newly launched LLM GPT-4o~\cite{ref:gpt4o} costs €0.0047 per 1,000 tokens, half the price of the GPT-4-Turbo, the model used in our experiment. Unfortunately, we could not test GPT-4o as it was launched too late for our study.

\section{Summary} \label{sec:summary5}

This chapter aims to validate the APITestGenie tool through two distinct experiments, comprehensively analyzing the results.

The first experiment tested APITestGenie using 25 distinct inputs, each executed three times, generating 75 tests. Metrics like generation time, token usage, and test outcomes were collected. The tool successfully generated Typescript code in 74 out of 75 runs, increasing generation time with more input tokens. Of the generated test cases, 55.1\% passed, while 44.9\% failed, mostly due to semantic errors like hallucinations and incorrect assumptions. Validity improved to 80\% upon the usage of the three attempts strategy. Using RAG enhanced test validity and reduced input tokens for complex APIs.

The second experiment involved a practical validation through a presentation to Critical Techworks staff, followed by feedback. Participants, including developers and product managers, found the tool relevant and complete, with most agreeing it could speed up test creation. Concerns were raised about immediate integration and security, but over half indicated a likelihood of using the tool daily. Suggestions included adapting the tool to other technologies and improving data generation capabilities.

The discussion highlights the importance of good documentation and processes when using APITestGenie. The tool is compared to GitHub Copilot, noting APITestGenie’s advantage in autonomously generating integration tests. The use of RAG helps reduce hallucinations and improve transparency. Regarding the research questions, the model can generate both integration and fuzz tests. Compared to baseline results, APITestGenie offers enhanced creativity and autonomy, fewer data restrictions, adaptability to unique scenarios, reduced hallucinations, and increased knowledge context. To conclude, APITestGenie can accelerate the test development processes.

APITestGenie’s limitations include the LLM context window size, the need for expert validations, and high data processing costs. RAG helps mitigate the context window issue. The cost is expected to decrease as LLMs become more efficient.

Overall, the experiments confirm APITestGenie's robustness and usefulness, though improvements are needed in data security and reducing manual validation.

==> Tese_Andre/chapter5.tex <==
\chapter{Conclusion and Future Work} \label{chap:concl}

This chapter aims to wrap up the topics explored by discussing the main ideas obtained upon the development of APITestGeni. Section~\ref{sec:conclusion} synthesizes the project's key findings, contributions to the field, and practical implications. Section~\ref{sec:futurework} finalizes with a discussion about future work opportunities.

\section{Conclusion} \label{sec:conclusion}

API services are popular in the industry. They are easy to develop, deploy, and scale, making them one of the foundation components in modern applications. However, testing API services poses several challenges. In the literature, several techniques have been proposed for automatically generating test cases in many different testing contexts. To the best of our knowledge, there is no known technique capable of automatically producing integration and fuzz tests for API services with a black-box approach that requires the input of an openAPI specification and business requirement in natural language.

The development and validation of APITestGenie demonstrates significant advancements in autonomous API test generation. The tool effectively puts into practice modern technologies and techniques, including LLMs and prompt engineering. The experimental results showed that APITestGenie could successfully generate a test script code in the majority of the runs, with a notable improvement in test validity when utilizing appropriate business requirement descriptions, tree of thoughts, and RAG techniques. Furthermore, practical validation through industry feedback underscored the tool's relevance and potential to streamline the test creation process despite identified areas for improvement, such as test integration challenges and data security concerns.

APITestGenie provides a significant contribution to the field of software testing. Autonomously generating API tests addresses a critical bottleneck in the development lifecycle, which could reduce the time and effort required for test creation. The integration of LLMs highlights the potential of advanced AI technologies in practical applications. The tool's modular architecture provides a flexible and adaptable framework that can be extended to various testing scenarios.

The practical implications of APITestGenie are substantial for development teams and organizations. The tool's ability to autonomously generate and refine API tests can lead to significant efficiency gains, reducing the dependency on manual test creation and expert validations. The prototype showcases the feasibility of integrating APITestGenie into existing workflows, potentially accelerating the adoption of automated testing practices. However, the feedback from industry professionals highlights the necessity of addressing security concerns to ensure the data security and integrity of the organizations.

\subsection{Key contributions}

The key contributions of this thesis are the following:
\begin{enumerate}
    \item Analysis of the state of the art with improvement suggestions on existing tools.
    \item Technique to overcome LLMs context size constraints using RAG to process knowledge data.
    \item Guidelines to use when creating LLM prompts for test generation.
    %\item Validation of a practical and complex use case using LLMs.
    %\item Tool that accelerates the process of API test creation.
    %\item Working and validated tool for industry adoption.
    \item Tool validated in a real industry use case that is currently being adopted by the company to improve the internal validation processes of APIs.
    \item Scientific paper with main contributions.
\end{enumerate}

%Analise do estado de arte e improvement sobre ferramentas atuais
%Ferramente funcional e validada para uso da empresa.
%Acelera os processor de geração de testes.
%Validação de caso de uso complexo de LLMs.
%RAG applicability in API specification summarization.
%Guidelines when creating prompts for test generation.
%Artigo cientifico

%Key findings
%Contribution to the field
%Practical implications

\section{Future Work} \label{sec:futurework}
Generative AI has experienced significant advancements in recent years. Every month, new LLMs with unique capabilities become available. In this evolving landscape future work should focus on exploring the benefits of using more cost-effective LLMs with enhanced capabilities to meet the industry's needs. For our specific case, testing a model with a higher context window, such as Gemini, would be beneficial due to the knowledge-intensive nature of our work. 

Another relevant experiment would be to explore the benefits of fine-tuning an LLM with company-specific data, providing the model with a deeper business context. Exploring the use of open-source distributed LLMs, such as LLAMA3, could reduce costs and offer greater control over data management, enhancing privacy.

In this study, we used the default parameters when querying ChatGPT. Future work should consider tuning some parameters, such as temperature and top\_p, to potentially reach a higher amount of valid test scripts.

Additionally, making the tool more generic and adaptable to other technologies presents an opportunity for future development, broadening its applicability and utility. An agent-based approach could be explored. A set of functions could be defined using function-calling methods, enabling the LLM to use external tools effectively. Furthermore, parsing the entire API specification would allow the definition of functions for each resource, effectively improving interactions with the API.

Lastly, we aim to complete the scientific article synthesizing the results obtained from this research, providing a comprehensive overview of our findings.


==> Tese_Andre/quote.tex <==
\cleardoublepage
\thispagestyle{plain}

\vspace*{8cm}

\begin{flushright}
   \textsl{``Artificial intelligence is not a substitute for human intelligence; \\
           it is a tool to amplify human creativity and ingenuity.''} \\
\vspace*{1.5cm}
           Fei-Fei Li
\end{flushright}

